UCoDe: Unified Community Detection with Graph Convolutional Networks

Community detection finds homogeneous groups of nodes in a graph. Existing approaches either partition the graph into disjoint, non-overlapping, communities, or determine only overlapping communities. To date, no method supports both detections of overlapping and non-overlapping communities. We propose UCoDe, a unified method for community detection in attributed graphs that detects both overlapping and non-overlapping communities by means of a novel contrastive loss that captures node similarity on a macro-scale. Our thorough experimental assessment on real data shows that, regardless of the data distribution, our method is either the top performer or among the top performers in both overlapping and non-overlapping detection without burdensome hyper-parameter tuning.

==> content/4.old-solution.tex <==
\ia{Here we describe our model, \ourmethod, that integrates the simplicity of single-objective community detection with the power of combined scores, by introducing a new contrastive cross-entropy loss.
We propose a contrastive differentiable unsupervised clustering function that optimizes the modularity of the network.}

\ia{\ourmethod has three main components (1) a  \emph{GCN architecture} that computes the community assignment matrix $\cmat$, (2) a \emph{contrastive modularity loss} function to learn the parameters of the model, and (3) a generator of corrupted graphs for the contrastive loss.
}

\ia{\subsubsection{GCN architecture.} The main purpose of the GCN is to compute the community assignment matrix $\cmat$ using structure and node attribute information. 
Our architecture is a two-layer GCN~\cite{kipf2017GCN}: 
\begin{equation}
GCN(\hat{\adj},\xmat) = \texttt{ReLU}(\hat{\adj}\cdot\underbrace{\texttt{SeLU}(\hat{\adj}\xmat\wmat^{[0]})}_{\xmat^{[1]}}\wmat^{[1]})
\label{eq:model}
\end{equation}
\textcolor{blue}{where we use $\texttt{SeLU}$~\cite{Klambauer2017activation} and $\texttt{ReLU}(\xvec)=\max(0, \xvec)$ as non-linear activation functions in first and second layer respectively. }

The last layer of our GCN outputs community assignment probabilities through the \texttt{softmax$(\xvec)_i=\frac{e^{\xvec_i}}{\sum_j e^{\xvec_j}}$} activation function. 
\begin{equation*}
\cmat = \texttt{softmax}(GCN(\hat{\adj}, \xmat))
\end{equation*}

This architecture, although simple, allows for propagating information over the entire graph, thus capturing relationships within the graph's structure and the nodes' attributes. 
% \textbf\bigskip
% \textbf{Encoder for soft cluster assignment and node representation} Both encoders of our models are two layers Graph Convolutional Network (GCN) model (Kipf \& Welling)\cite{kipf2017GCN}. 
% The CoDe-GCN encoder is as follows: 

% \begin{equation}\label{eq:Encoder2}
%     GCN (X,A)= \hat{D}^{-1/2}\hat{A}\hat{D}^{-1/2}X\theta
% \end{equation}
% \begin{equation}
%     H_1=\sigma(GCN (X,A))
% \end{equation}
% \begin{equation}
%     \mathcal{E}(X,A)=\sigma(GCN (H_1,A))
% \end{equation}


% where  $GCN$ is defined in equation (\ref{eq:Encoder2}). The activation function of the first layer of soft cluster assignment is ReLU. The activation function of the first layer of node representation is SELU. The activation function for the second layer of both models is ReLU. $\hat{A}=A+I_N$ is the adjacency matrix with self-loops, and $\hat D_{ii}=\sum_{i}\hat A_{ij}$ is the diagonal matrix of 
% $\hat A$. \bigskip
}
% In this section we will present our method, \ourmethod that considers both attributes and structure of the graph for detecting the communities. Our model is inspired by the modularity function.

%\subsection{\ourmethod} 
% We proposed a GNN-based approach that optimizes the modularity in the network by utilizing the contrastive type objective function. We proposed two encoders with the same objective functions. One encoder generates the cluster assignments of the nodes. The other encoder generates node representations for the graph. The proposed contrastive objective function is fully differentiable and optimizes both soft clustering and node representations in an unsupervised manner.


%%% This is NOT our objective - this is our method. 
% our objective is to learn two encoders:

% first, $\mathcal{E}: {\mathbb{R}^{N \times F}} \times {\mathbb{R}^{N \times N}} \overrightarrow{} {\mathbb{R}^{N \times F'}}$ such that $E(X,A)=H=\{\vec{h_1},\vec{h_2},\vec{h_3}...,\vec{h_N}\}$ represents high-level representations $\vec h_i \in \mathcal{R^{F'}}$ for each node $i$. These representations are used for detecting communities in the graph.

% Second, $\mathcal{E}: {\mathbb{R}^{N \times F}} \times {\mathbb{R}^{N \times N}} \overrightarrow{} {\mathbb{R}^{N \times F'}}$ such that $E(X,A)=H=\{\vec{h_1},\vec{h_2},\vec{h_3}...,\vec{h_N}\}$ represents the  associated probability  $\vec h_i \in \mathcal{R^{F'}}$ for each node $i$ to communities. 




\ia{\subsubsection{Contrastive modularity loss}
The GCN loss function is crucial in describing the properties that communities detected by the model will have. As discussed above, a GCN that maximizes only modularity as a single score inherits its limitations, such as a tendency to favor overly small communities. Combining many loss functions, on the other hand, results in a brittle model where parameter tuning quickly becomes an intricate process.

We propose a contrastive loss that mitigates these shortcomings by contrasting node representations from the input graph with those computed on a corrupted graph $\widetilde{\Gr}$, where the latter should not show the same community structure. In this way, the GCN is encouraged to bypass representations that do not convey the community structure in the input graph. On the corrupted graph, the GCN outputs a corrupted assignment $\tilde{\cmat}$.

In the input graph, we define the vector $\mvec$ as 
\begin{equation*}
    \mvec= \Diag\left(\frac{{\cmat^\top}\bmat{\cmat}}{2|\E|}\right)
\end{equation*}
\blue{If we omit the rewiring part, the $\tilde{m}$ formula should be revised}
Analogously for the corrupted graph, we define $\widetilde{\mvec}$ as
\begin{equation*}
    \widetilde{\mvec}=\Diag\left(\frac{\tilde{\cmat}^\top \bmat\tilde{\cmat}}{2|\E|}\right)
\end{equation*}
Intuitively, vector $\mvec$ ($\tilde{\mvec}$, respectively) represents the relative density of each of the communities in the input (corrupted, respectively) graph. 

To compute our objective, we transform community detection into a classification problem in which the model learns how to discriminate real communities from corrupted communities.

Given an indicator variable $\yvec$ such that $\yvec_i = 1$ if $i$ is a community from the input graph, and 0 otherwise, \ourmethod's loss function is
% In order to optimize the cluster assignment matrix the following objective function is proposed. The proposed objective function optimizes modularity through contrastive operation. For optimization,  we use a noise-contrastive type objective with a standard binary cross-entropy (BCE) loss between the samples from the positive examples and negative examples. The proposed objective function is as follows:

\begin{equation}
\mathcal{L}_{\ourmethod}=-\frac{1}{2k}\left( \sum _{i=1}^{k} \yvec_i \log ({\mvec}_i) + \sum _{i=1}^{k} (1-\yvec_{i}) \log (1-\widetilde{\mvec_i})\right)
\label{eq:objective}
\end{equation}
Note that the loss promotes representations for which the modularity is high in the input graph rather than in the corrupted one. Figure~\ref{fig:modularity} demonstrates this difference in the modularity score of a real vs corrupted graph as learning evolves.

Please note that Eq.~\ref{eq:objective} is fully differentiable since it is the composition of differentiable functions, and is therefore amenable to gradient descent optimizers, such as Adam~\cite{kingma2014adam}.
% Where $k$ is the number of communities, $\tilde{k}$ is the number of communities of negative samples. \dm{In our case,} the number of communities in both negative and positive samples is equal. $H$ is the representation of positive samples and $Mod(H)$ is obtained from {refer to equation 9}.  $Mod(\tilde{H})$ is the y is the true class of the modularity of each community. The $y_i$ is 1 for the modularity of the positive samples. $y_i$ is 0 for the modularity of the negative samples.
%\input{figs/fig-modularity}     
}

\subsubsection{Generating the corrupted graph.} \ia{The generation of the corrupted graph $\tilde{\Gr}$ is fundamental to obtaining good node representations. 

A corrupted graph that still remains too similar to the input graph $\Gr$ would not provide the necessary contrast. Technically, it would have a negative impact on the loss in Eq.~\ref{eq:objective} by collapsing the representations of the two graphs. On the other hand, a corrupted graph that bears almost no similarity to the input graph would not carry enough community structure to allow the GCN to capture relevant differences in learning the representations. 


\textcolor{blue}{Should we omit Rewiring part? We can also keep it but we use Andrew's explanation to prove that shuffling is a better choice}

In order to obtain corrupted graphs that exhibit adequate contrast to the input graphs, we propose two strategies. They take outset in graph-theoretical intuitions and the design of our loss function. 

%We introduce two strategies for generating negative samples.

\begin{enumerate}
    \item \textbf{Rewiring}: we rewire the graph such that we still retain the degree of each node $\dg_i$, but choose $\dg_i$ nodes in the graph uniformly without replacement to connect to. Such a rewiring process is theoretically studied in models such as the Watts-Strogatz graph generator~\cite{watts1998collective}.
    \item \textbf{Shuffling}: we permute uniformly at random the vector $\mvec$ in the original graph. This process retains the overall modularity score $Q$, but tends to generate communities with distorted densities, informing the loss function to preserve densities. 
\end{enumerate}
}


\subsubsection{Overview of \ourmethod} 
\ia{Finally, we provide an overview over the major steps in \ourmethod. The algorithm generates  representations through our trainable architecture in Eq.~\ref{eq:model} and the loss function in Eq.~\ref{eq:objective}, to return soft cluster assignments $\cmat$. 
The overall process is the following:

\begin{enumerate}
    \item Compute the soft cluster assignment $\cmat$ for the input graph, training the GCN model in Eq.~\ref{eq:model}.
    \item Compute the soft cluster assignment $\tilde{\cmat}$ for the corrupted graph using the same model as in step (1).
    \item Compute vector $\mvec$ for the input graph, and vector $\tilde{\mvec}$ for the corrupted graph.
    \item Update the parameters of the $GCN$ model via gradient descent to minimize the loss function in Eq.~\ref{eq:objective}.
\end{enumerate}


} 




% Below we give an overview of \ourmethod. In the following setup we give an overview of the steps of soft cluster assignment for each nodes. Moreover, we use the first negative sample generation startegy (generating corrupted graph) 





==> content/old/0.abstract.tex <==
%!TEX root=../main.tex
\begin{abstract}
% \cmt{9 pages incl. refs + 2 pages supplementary}

\ia{Community detection is the unsupervised task of finding \dmk{homogeneous groups of nodes in a graph}. Existing approaches  \dmw{either partition the graph in disjoint, \emph{non-overlapping}, communities, or return \emph{overlapping} communities. \dmk{To date}, no method satisfactorily detects both overlapping and non-overlapping communities.} 

\dmw{We propose \ourmethod, a \emph{unified} method for unsupervised community detection in attributed graphs which leverages recent developments in Graph Neural Networks (GNNs) for representation learning.
So far, GNN methods for community detection provide competitive results in either overlapping or non-overlapping community detection tasks, but have had little success in both.}
\ourmethod overcomes these issues by introducing a new loss that captures node similarity on a macro-scale. 
\dmk{Our thorough experimental assessment on real data shows that, without prejudices on the data distribution, our method is either the top performer or among the top performers in both overlapping and non-overlapping detection, without burdensome hyper-parameter tuning. As a further point, we provide theoretical insights on the model's characteristics.}}

% theoretical justification for our approach's validity in the task of community detection and show that it can be applied in both the overlapping and non-overlapping settings. As our experiments demonstrate on several real benchmark graphs, \ourmethod consistently provides high-quality results in both overlapping and non-overlapping settings in an easy to apply fashion.}}


% have shown tremendous promise in graph-related tasks. However, they have received less attention in detecting communities in the graph. In this paper, we study GNNs potential in detecting communities in an unsupervised manner.

% We present CoDe-GCN, an unsupervised contrastive type Graph Convolutional Neural Network model for detecting communities in the graph-structured data. The core idea of our model is to find the communities in the network by considering the modularity measure. Detecting communities using modularity measure is a traditional approach; however, finding communities by considering this measure is an NP-hard problem. To tackle it, we start by drawing a connection between GNNs and Modularity measures as an objective function. There have been a few works that used GNNs and derived communities by optimizing the Modularity measure. In contrast to previous works, CoDe-GCN finds the communities in the network by training a contrastive type objective function to derive the communities that increase the network's modularity.  We show that our model detects high-quality communities compared to the state-of-art of models.






\end{abstract}

==> content/old/1.introduction.tex <==
%!TEX root=../main.tex
\section{Introduction}\label{sec:introduction}


\ia{Community detection~\cite{fortunato2010community} is the problem of identifying sets of nodes in a graph that share common characteristics. 
In social networks, community detection identifies groups of individuals who participate in joint activities, such as sports clubs, or have similar preferences~\cite{perozzi2014deepwalk}; in biological networks, community detection can automatically identity proteins that contribute to a specific disease~\cite{mall2017adaptive}. 
\aad{Such networks include information in node attributes that may be helpful when identifying similarities (e.g., the age of a person).}
\dmw{However, these attributes are often disregarded} by traditional community detection methods, such as spectral clustering~\cite{shi2000normalized}, modularity maximization~\cite{newman2006modularity}, or more recent graph embeddings~\cite{cai2018comprehensive}, making them ill-suited for detecting node communities in \dmw{attributed} graphs.}%\ccmt{Isn't it better we change the heterogeneous?}

\ia{In recent years, graph neural networks (GNNs)~\cite{kipf2017GCN, velivckovic2018deep, hamilton2017inductive, bronstein2017geometric, battaglia2018relational} have shown superior performance in a number of supervised tasks on graphs, especially link prediction, node classification, and graph classification. 
GNNs' popularity stems from their aptitude to capture complex relationships in networks, typically by means of propagating node attributes and features to neighboring nodes by a message-passing process~\cite{battaglia2018relational}. \aad{These are typically accompanied with a 
\emph{graph pooling}~\cite{bruna2014spectral,bianchi2020spectral,lee2019self} method, which aggregates multiple nodes into higher-level representations with the aim of reducing the number of parameters of the neural network.}}
%Pooling algorithms thus produce intermediary layers in the GNNs and do not explicitly return communities.}

\ia{GNNs have propelled advancements in supervised tasks\dmw{; yet on} unsupervised tasks such as community detection, \dmw{GNNs have attained significantly fewer prominent results.}
Most existing GNN methods do not directly optimize for community detection but achieve the objective indirectly.
Unsupervised GNNs, such as the popular Deep Graph Infomax (DGI)~\cite{velivckovic2018deep}, find node representations that need to be subjected to a clustering algorithm, such as k-means, to obtain communities. 
}

\ia{Recently, a few methods propose GNNs that \emph{explicitly} optimize for community detection. 
\dmw{GNNs for \emph{non-overlapping} community detection}
either optimize \dmw{for} a \emph{single score} or \emph{combine several scores}. \dmw{Single score} methods revisit traditional measures such as min-cut~\cite{bianchi2020spectral} and modularity~\cite{tsitsulin2020graph} objectives to return node-community probabilities. Combined score methods~\cite{zhang2019attributed, zhang2020commdgi} integrate multiple different objectives. \dmw{These methods outperform single score methods in non-overlapping community detection, but} they require substantial tuning to the dataset at hand and are typically less robust and less interpretable than their single objective counterparts.  \dmw{Non-overlapping community detection aims at returning a single community assignment for each node. As such, they are ill-suited for overlapping community detection.} 
\dmw{NOCD~\cite{shchur2019overlapping} is, at the time of writing this paper, the only GNN that optimizes  for \emph{overlapping community} detection. In particular, NOCD finds communities that maximize the probability of recovering the graph structure. Yet, this approach constrains the community structure to be overlapping. In conclusion, to date no GNN can seemingly detect overlapping and non-overlapping communities. 
}

% However, these objectives carry the problems of the scores they optimize; for instance, modularity encourages small communities when the number of communities is high~\cite{lancichinetti2011limits}. 


%Therefore, while single objective methods might not discover the right communities, combined objective methods require a significant amount of tuning on the different datasets.
}

\ia{\spara{Our method.} We propose \ourmethod, a GNN for community detection with a single loss \dmk{based on network \emph{modularity}} while \dmw{explicitly allowing overlaps among communities}. \dmk{We devise a novel contrastive loss} that attains \dmk{overall} superior results by comparing the real network with one in which the communities are shuffled.
Our loss function \dmw{encourages a clean community structure without discouraging overlapping communities. We provide theoretical \dmk{insights} for this choice as well as experimental evidence.}
%discourages overly small or overly large communities via negative sampling of the corrupted networks that likely expose no community. 
%To generate corrupted networks we propose two graph-theoretic strategies. 
\dmk{We show that our model achieves competitive results than methods explicitly designed for either overlapping or non-overlapping community detection with an end-to-end model that requires minimal hyperparameter tuning.}}

%We show that our model achieves better results than single objective methods on community detection and comparable performance to combined objective ones with a much simpler model that overcomes the need for extensive tuning.}

\ia{\spara{Contributions.} In summary, our contributions are as follows.

\begin{itemize}[leftmargin=*]
    \item We introduce a new GNN, \ourmethod, for community detection on graphs (Section~\ref{sec:solution}). We leverage state-of-the-art representations and devise a simple, effective single score model.  
    \item \ourmethod uses a new contrastive loss that promotes both overlapping and non-overlapping communities, achieving competitive results across contexts with the same model (Section~\ref{sec:solution}). 
    \item We perform extensive experiments on real data, showing that our method outperforms single objective methods while more easily achieving quality on par with more complex combined scores (Section~\ref{sec:experiments}). %\ccmt{I think it is better we omit the synthetic because we don't show any results.}
\end{itemize}}



==> content/old/2.related-work.tex <==
%!TEX root=../main.tex

\input{tables/tbl-related-work.tex}

\section{Related Work}\label{sec:related-work}


\ia{Before delving into our solution, we provide an overview of the literature on \dmw{community detection, graph neural networks, graph pooling, and graph embeddings}. Table~\ref{tbl:relatedwork} provides a summary of the characteristics of the most important work in the area. 


\subsection{Community detection}
\ia{Community detection has a long history in graph analysis~\cite{fortunato2010community} with applications across the natural sciences. 
There are two main categories of community detection: \textit{non-overlapping} community detection, also called partitioning, seeks an assignment of each node to exactly one community; \textit{overlapping} community detection, seeks a soft-assignment of nodes into potentially multiple communities. 
A community detection algorithm optimizes a score that describes the cohesiveness of nodes in the community with respect to the rest of the nodes. 
%Here we focus on the more fundamental problem of non-overlapping community detection. 
A number of scores and methods have been proposed, such as spectral clustering for min-cut~\cite{shi2000normalized}, Louvain's method for modularity~\cite{newman2006modularity}, and the Girvan-Newman algorithm for betweenness~\cite{Girvan_2002/betweeness}. Overlapping community detection is often approached using algorithms similar to the Expectation-Maximization algorithm for soft-clustering~\cite{dempster1977maximum} where each point is a distribution over the clusters. Similarly, AGM~\cite{yang2012community} and BigCLAM~\cite{yang2013overlapping} formulate the community detection problem as finding soft-assignments to communities that maximize the model likelihood.  {EPM}~\cite{zhou2015infinite} is based on Bernoulli–Poisson models, {SNMF}~\cite{SNMF2010} and {CDE}~\cite{CDE2018} use non-negative matrix \dmw{factorization.}
} 


\subsection{Graph Neural Networks}
GNNs~\cite{wu2020comprehensive} are a family of parametric models that learn node representations by aggregating features over the graph's structure. 
As such, they are particularly apt for representing information in attributed graphs. 
GNNs are extremely flexible models that exhibit state-of-the-art performance on a number of \emph{supervised tasks}, such as link prediction, node classification, and graph classification.

Popular GNN models include spectral GNNs~\cite{bronstein2017geometric, defferrard2016convolutional}, GCNs~\cite{hamilton2017inductive,kipf2017GCN}, graph autoencoders (GAEs)~\cite{kipf2016variational}, isomorphism-based networks~\cite{xu2018powerful}, and DGI~\cite{velivckovic2018deep}. These models compute node features in an unsupervised manner if equipped with a reconstruction loss. A clustering algorithm, such as k-means, can cluster the node features to return communities. Since there is no coupling between such GNN model objectives and the clustering algorithm, the resulting communities may not accurately represent all groups in the graph.  

\spara{GNNs for community detection.} Some GNNs directly optimize for non-overlapping community detection with community-wise loss functions. \emph{Single objective} approaches propose variations of traditional cohesiveness scores, such as min-cut~\cite{bianchi2020spectral} and modularity~\cite{tsitsulin2020graph}. \dmw{Yet, single-objective methods inherit the limitations of the score they aim to optimize, providing community memberships that are subject to the loss objective's definition of community.} 
%For more details, see the discussion at the end of Section~\ref{ssec:modularity}.
CommDGI~\cite{zhang2020commdgi} proposes a \emph{combined objective} as a linear combination of three objectives, the DGI objective~\cite{velivckovic2018deep}, modularity, and mutual information. CommDGI's combined objective overcomes the limitations of the single score methods, but requires extensive parameter tuning for proper results. \dmw{Although models like DMoN~\cite{tsitsulin2020graph} return soft community assignments through a softmax output layer, both single and combined objective methods explicitly penalize overlaps among communities. 

NOCD~\cite{shchur2019overlapping} proposes an overlapping community detection loss that maximizes the likelihood on Bernoulli-Poisson models~\cite{shchur2019overlapping}. NOCD achieves competitive results on overlapping community detection but cannot directly detect non-overlapping communities.}
}
%DM: Aug 12



% DM: Old-text

% \spara{Combined-objective GCNs:}
% Multi-objective boosts the performance, but the tuning becomes harder. 

% CommDGI~\cite{zhang2020commdgi}, generates clustering assignments by maximizing the combination of objective functions. The objective function in this model is a combination of three objective function. First, modularity quality of the cluster. Secondly, mutual information mechanism between nodes and graph structure. Third, community representation for each node.

% \spara{Single-objective:}
% Several unsupervised training of GCN models has been proposed that detect communities in the network. DMoN~\cite{tsitsulin2020graph}, is a clustering assignment method that trains a GCN in an unsupervised manner by maximizing the modularity. 
%AGC is an adaptive graph convolution method for
%attributed graph clustering that exploits high-order graph
%convolution to capture global cluster structure and adaptively selects the appropriate order for different graphs.%


% Table\ref{} gives an overview of five desirable properties of graph clustering methods with graph neural networks. 
% \begin{itemize}
%     \item \textbf{Unsupervised } methods learn the communities without using the ground truth in the learning procedure.
%     \item \textbf{Trainable} methods are able to learn the objective function step-by-step.
%     \item \textbf{Modularity-based} methods detect the community by optimizing the modularity function.
%     \item \textbf{Contrastive-type} methods are an important approach for unsupervised learning of representations. This method train the method to be contrastive between the representations that capture the dependencies of interest and those that do not.
%     \item \textbf{Soft assignments } provides a probability of nodes belongings to each cluster.
%     \item \textbf{Single Objective}: The method only optimize one objective function. CommDGI~\cite{zhang2020commdgi} optimizes objective function consists of several different objectives.
% \end{itemize}








\subsection{Graph Pooling}

% Used internally to simplify the network / equivalent to the pooling operator in Neural Networks 
\ia{Graph pooling~\cite{bruna2014spectral,bianchi2020spectral,lee2019self} is an operation that aggregates nodes so as to learn summarized representations. 
The purpose of graph pooling is to remove redundant information and reduce the number of parameters of the GNN. 

\emph{Model-free pooling} coarsens the graph structure by aggregating nodes without considering the node attributes. Graclus~\cite{dhillon2007weighted} revisits max-pooling to aggregate similar nodes in a hierarchical fashion. SAGPool~\cite{lee2019self} proposes a self-attention layer to reweigh nodes in the graph. Model-free approaches act as layers in the network and do not provide communities as output. 

\emph{Model-based} pooling learns coarsening operators through a differentiable loss function. DiffPool~\cite{Ying2018diffpool} learns a hierarchical clustering assignment of the graph for supervised graph classification. Top-K pooling~\cite{Ga02019TopK} trains an autoencoder that assigns a score to each node; the pooling phase retains the k nodes with the highest score. Yet, these methods do not explicitly optimize for cluster assignments resulting in substandard communities~\cite{bianchi2020spectral}. MinCutPool~\cite{bianchi2020spectral}, although a pooling technique, returns community assignments by optimizing the min-cut objective of spectral clustering~\cite{shi2000normalized}. MinCutPool does not require eigendecomposition of the Laplacian matrix, and instead propagates node attributes over the GNN. 
%  solves the same objective as spectral clustering with the use of an MLP. Specifically, they represent the problem of finding the minimum cut as an unsupervised loss function and train the MLP to output a cluster assignment matrix.  
}


\subsection{Node embeddings}
\ia{Node embeddings~\cite{cai2018comprehensive,chami2020machine} learn node representations of the graph structure in an unsupervised manner with shallow neural networks~\cite{perozzi2014deepwalk, tang2015line}, autoencoders~\cite{wang2016structural}, or matrix factorization~\cite{ou2016asymmetric,qiu2018network}. Similar to GNNs, a clustering algorithm on the embeddings can detect communities. Node embeddings can be seen as a generalization of dimensionality reduction methods, and tend to preserve the structure but disregard node attributes. A few recent works address the problem of attributed node embeddings through matrix factorization~\cite{yang2015network} or deep model DANE~\cite{gao2018deep}. \dmw{None of these models are designed for community detection. AGC~\cite{zhang2019attributed} proposes a spectral filter for community detection that seemingly applies to \emph{any} GNN to improve their performance.}
%AGC first applies a spectral filters on the node attributes using the k-th power of the graph's Laplacian matrix and then use spectral clustering on the similarity matrix obtained by pairwise dot-product of the filtered node attributes.
}
% utilize the graph pooling operation to learn more abstract and coarser representations of the input graphs by summarizing local components and discarding redundant information.

% There are two main families of graph poolings in GNN. First, Model-free and second, Model-based pooling. The Model-free pooling methods pre-compute the coarsened graph based on graph structure and they don’t consider the node features explicitly. Graclus~\cite{2016DefferrardGraclus} is a Model-free based method. 

% In Graclus~\cite{2016DefferrardGraclus}, similar nodes will be clustered together hierarchically. A max-pooling operation is used in GNN to determine the node’s attributes. 

%Second, Model-based pooling methods learn to coarsen the graph through learnable functions. 






 
%\cmt{DM note: Talk about overlapping community detection}

% Uncomment this part if we have overlapping community detection.  






% \subsection{Graph embeddings}

% Deep Graph infomax~\cite{velivckovic2018deep},  produces low-level graph representation by learning the nodes' representations in an unsupervised manner. The model uses a contrastive type loss function by maximizing the mutual information of nodes and graph structure. 

% AGE\cite{Cui2020AdaptiveGE} is an adaptive graph embedding method that utilize non-parametric Laplacian smoothing instead of graph convolution neural networks.


% We can refer to the traditional algorithms such as Modality Maximization~\cite{Newman_2006}, Louvain's method ~\cite{DBLP:journals/corr/abs-1108-1502/Louvain}, betweenness centrality~\cite{Girvan_2002/betweeness} that were proposed for non-overlapping community detection.  Later new methods such as hierarchical clustering of the edges~\cite{Ahn_2010hierarchical}, Community Affiliation Graph model~\cite{6413734/Affiliation} and Bigclam~\cite{yang2013overlapping/bigclam} have been proposed for overlapping community detection.

% In general, types of community detection can be divided into overlapping community detection, where one node can have multiple community membership in the network, and non-overlapping community detection, where the network can be partitioned into subgraphs and nodes in each subgraph have more connections amongst each other. 
  









% Non-linear Dimensionality reduction on matrix




==> content/old/3.preliminaries.tex <==
%!TEX root=../main.tex
\vspace{-2mm}
\section{Modularity \& GNNs}\label{sec:main}
\ia{%In this section, we describe our approach for contrastive community detection. 
We review graph community detection and discuss the modularity loss before presenting our Unified Community Detection (\ourmethod).}

\subsection{Preliminaries and Problem}\label{sec:preliminaries}
% In this section, we will present the necessary background for \ourmethod. First, we will explain the problem formulation, then we will explain the methods that motivated CoDe-GCN objective function.\smallskip
\ia{Consider an \emph{attributed graph} $\Gr = (\V, \E, \A)$ where $\V = \{v_1, .., v_\nn\}$ is a set of $\nn$ nodes, $\E \subseteq \V \times \V$ is a set of edges and $\A = \{a_1, ..., a_\na\}$ is set of $\na$ attributes. Each node $v_i$ has an associated vector $\xvec_i \in \reals^\na$ of real features for each attribute. 
The node features form a ${\nn \times \na}$ matrix $\xmat \in \reals^{\nn \times \na}$ where each node-feature vector $\xvec_i$ is a \dmw{row in such matrix.} 
The \emph{adjacency matrix} is a matrix representation  $\amat$ of the graph's structure, where $\amat_{ij} = 1$ if $(v_i,v_j) \in \E$, and $0$ otherwise. The \emph{degree} $\dg_i$ of a node $v_i$ is the number of neighbors of node $i$, i.e., $\dg_i = \sum_{j=0}^\nn \amat_{ij}$; $\dgvec$ is the vector containing the degree $\dgvec_i=\dg_i$ of all nodes, and $\dgmat$ is the diagonal degree matrix.}

\ia{\spara{Attributed graph community detection.} We aim to assign each node to at least one of $k$ communities, $\Cl_1, ..., \Cl_k$, such that \dmk{a score of \emph{community cohesiveness} is maximized.} The cluster assignment is a probability vector $\cvec_i$ indicating the probability $c_{ij} = p_{ij}$ of node $v_i$ belonging to community $\Cl_j$. \dmw{Cluster assignments form a matrix $\cmat \in [0,1]^{\nn \times k}$ where row $i$ is the cluster assignment $\cvec_i$ for node $i$.}}

\smallskip
\ia{One of the determinant choices for community detection algorithms is the definition of the community cohesiveness score that determines the quality of the cluster assignments. In the following, we review modularity~\cite{newman2006modularity}, a popular measure for community detection, and discuss the limits and pitfalls of its direct maximization.} 



% We assume that we have a graph $G$ with a set of node features, $\textbf{X}=\{\vec{x_1},\vec{x_2},\vec{x_3},...,\vec{x_N}\}$ where $N$ is the number of nodes in the graph and $x_i\in \mathbb{R}^F$ are the features of node $i$. The relational information between these nodes are represented by the adjacency matrix, $A\in \mathbb{R}^{N\times N} $. We also assume that the graph is unweighted, then $A_{ij}=1$, if there exists an edge between node $i$ and $j$, otherwise $A_{ij}=0$.

\vspace{-2mm}
\subsection{Modularity}\label{ssec:modularity}

\ia{\emph{Modularity}~\cite{newman2006modularity} is a measure $Q(\Gr;\Cl)$ of quality of a partition $\Cl$ of the nodes of the graph $\Gr$. High values indicate groups with dense internal connections and sparse connections to outside nodes.
The modularity is defined as the difference in density between the edges inside a community $\cvec_i$ and the edges of a fixed null model. 
The null model in the modularity score is the rewiring model, in which each node $v_i$ preserves its degree $\dg_i$ but connects randomly to any other node in the graph.
The modularity score is 
\begin{equation}\label{eq:modularity1}
    Q(\Gr;\Cl)=\frac{1}{4|\E|}\sum_{s=1}^k\sum_{ij}\left(\amat_{ij}-\frac{{\dg_i}{\dg_j}}{2|\E| }\right)\cmat_{is}\cmat_{js}
\end{equation}

\noindent The quantity $\frac{{\dg_i}{\dg_j}}{2|\E| }$ is the null-model representing the probability that two nodes $v_i, v_j$ are connected by chance. 
The modularity when $k=2$ is a number $Q(\Gr; \Cl)\in (1/2;1]$. 
By defining the \emph{modularity matrix} $\bmat$ as $\bmat_{ij} = \amat_{ij}-\frac{{\dg_i}{\dg_j}}{2|\E|}$, the modularity in Eq.~\ref{eq:modularity1} simplifies into

\begin{equation}\label{eq:mod_matrix}
    Q(\Gr;\Cl)=\frac{1}{4|\E|}\tr(\cmat^\top\bmat\cmat)
\end{equation}

\noindent We can write $\tr(\cmat^\top \bmat\cmat)$ as sparse matrix multiplication
\begin{equation}\label{eq:sparse_modularity}
\tr(\cmat^\top \adj\cmat-\cmat^{\top} \dvec \dvec^{\top} \cmat)
\end{equation}

A modularity close to $1$ denotes a good partition of the graph. As such, several community detection algorithms aim to maximize modularity to detect communities. Modularity maximization is an \NPhard problem, solved with approximate methods, such as the Louvain greedy algorithm~\cite{blondel2008fast} and the spectral modularity~\cite{newman2006modularity}.%, or hierarchical methods~\cite{clauset2004finding}. 
% The direct maximization of modularity is $\NPhard$
% The above mentioned matrix is called the modularity matrix. The properties of this function are used for modularity optimization. The elements of its rows and columns are equal to zero. Therefore it always has an eigenvector(1,1,1,..) with eigenvalue zero. This graph has a similar characteristic to graph Laplacian, which is the basis for many clustering algorithms such as spectral clustering and graph partitioning. For community detection, modularity should be maximized. Since finding global maximum is an \textbf{NP-hard} problem, several optimization methods, such as spectral modularity maximization~\cite{Newman_2006}, Clauset et al.~\cite{PhysRevE.70.066111Clauset}, Duch and Arenas~\cite{Duch} are proposed.
}

\dmw{
\mpara{Limits and pitfalls.} Modularity maximization is one of the most popular methods for community detection~\cite{fortunato2010community}. However, its direct maximization may fail to provide optimal communities. \dmk{As has been noted in \cite{fortunato2007resolution}, the modularity may fail to recognize clusters that fall below a graph-specific size}. Furthermore, modularity is a measure for discrete partitioning and does not perform well in the case of overlapping communities. In Section~\ref{sec:solution}, we will show how to overcome this limitation of modularity by introducing a contrastive objective. %\cmt{I don't believe the second limitation is formally addressed in section 4}
}


\subsection{Modularity loss for GNNs}

\ia{The objective in Eq.~\ref{eq:mod_matrix} is \NPhard but can be solved efficiently with a spectral approach similar to spectral clustering~\cite{newman2006modularity} if we allow matrix $\cmat$ to be real, rather than binary. This relaxed objective admits as solutions the $k$ leading eigenvalues of the matrix $\bmat$. \dmw{This convenient relaxation enables soft clustering assignments and, in principle, overlapping community detection.}
\dmk{A recent, yet unpublished work, DMoN~\cite{tsitsulin2020graph}, allows for the matrix $\cmat$ to take the form of the output of a Graph Neural Network (GNN). To appreciate this coherent, but convenient, transformation, we first introduce the formalism of GNNs.}

\mpara{Graph Neural Networks}~\cite{kipf2017GCN, velivckovic2018deep, hamilton2017inductive, bronstein2017geometric, battaglia2018relational} are machine learning models that transform the node attributes by nonlinear aggregation of attributes of each node's neighbors. By virtue of this aggregation mechanism, these networks are called message passing~\cite{battaglia2018relational}. We now review the \dmw{Graph Convolutional Network (GCN) model~\cite{kipf2017GCN}.} % Why simple?  
We denote as $\xmat^{[0]}$ the initial node attributes $\xmat^{[0]} = \xmat$,  
\[\hat{\amat} = \dgmat^{-1/2}(\adj + \eye)\dgmat^{-1/2}\]  
the normalized adjacency matrix with self-loops, and $\wmat^{[t]}$ the weight matrix at layer $t$ which encodes the parameters of the network. 
The $t{+}1$ layer $\xmat^{[t+1]}$ is

\begin{equation*}
    \xmat^{[t+1]} = \sigma(\hat{\amat}\xmat^{[t]}\wmat^{[t]})
\end{equation*}

The function $\sigma$ is a non-linear activation function, such as softmax, SeLU, or ReLU. The matrix $\wmat^{[0]}$ is randomly initialized, typically as $\wmat^{[0]}{\sim}\mathcal{N}(0,1)$. The parameters $\wmat$ are learned via stochastic gradient descent on a supervised or unsupervised loss function.  

\mpara{DMoN}~\cite{tsitsulin2020graph} is a GCN that learns community assignments with a modularity-based loss function. 
The DMoN architecture integrates learnable features through a message passing mechanism with a modularity objective that pushes for community structure. In this way, the attributes are seamlessly integrated into the modularity score, and modularity informs the GCN on how to obtain representations that reflect communities.
The loss function consists of modularity maximization and a regularizer to ensure balanced communities. The DMoN objective function is as follows:

\begin{equation}\label{eq:dmon}
    \mathcal{L}_{\mathrm{DMoN}}=-\frac{1}{2 |\E|} \operatorname{Tr}\left(\cmat^{\top} \bmat \cmat\right)+\frac{\sqrt{k}}{n}\left\|\sum_{i} \cmat_{i}^{\top}\right\|_{F}-1
\end{equation} 

\noindent where $\|\cdot\|_F$ is the Frobenius norm. By using the sparse modularity in Eq.~\ref{eq:sparse_modularity}, DMoN allows for efficient parameter optimization.

\dmw{\mpara{Limits and pitfalls.} Note that the DMoN objective in Eq.~\ref{eq:dmon} explicitly penalizes overlapping communities. Indeed, the regularization term  $\frac{\sqrt{k}}{n}\left\|\sum_{i} \cmat_{i}^{\top}\right\|_{F}-1$ enforces sparsity of $\cmat$ and, thus, penalizes nodes assigned to multiple communities.} 


% DMoN~\cite{tsitsulin2020graph} derives a differentiable modularity objective for GNNs.

% soft cluster assignment for each node by proposing a differentiable objective function. 


% I should fix this --->
% \begin{equation}
%     {L_{DMon}}=-\frac{1}{2m} Tr({C^T}{B}{C})+ \norm { \frac{\sqrt{k}{n} }}
% \end{equation} 






% Graph Neural Networks are a flexible class of models that perform nonlinear feature aggregation
% with respect to graph structure. For the purposes of this work, we consider transductive GNNs that
% output a single embedding per node. Graph convolutional networks (GCNs) [29] are simple yet
% effective [51] message-passing networks that fit our criteria. Let X0 ∈ R
% n×s be the initial node
% features and A˜ = D− 1
% 2 AD− 1
% 2 be the normalized adjacency matrix, the output of t-th layer Xt+1 is
% Xt+1 = SeLU(AX˜ tW + XWskip) (3)
% We make two changes to the classic GCN architecture: first, we remove the self-loop creation and
% instead use an Wskip ∈ R
% s×s
% trainable skip connection, and, second, we replace ReLU nonlinearity
% with SeLU [30] for better convergence.

% \cmt{Davide: Add what is d and what is D}
}


==> content/old/4.old-solution.tex <==
\ia{Here we describe our model, \ourmethod, that integrates the simplicity of single-objective community detection with the power of combined scores, by introducing a new contrastive cross-entropy loss.
We propose a contrastive differentiable unsupervised clustering function that optimizes the modularity of the network.}

\ia{\ourmethod has three main components (1) a  \emph{GCN architecture} that computes the community assignment matrix $\cmat$, (2) a \emph{contrastive modularity loss} function to learn the parameters of the model, and (3) a generator of corrupted graphs for the contrastive loss.
}

\ia{\subsubsection{GCN architecture.} The main purpose of the GCN is to compute the community assignment matrix $\cmat$ using structure and node attribute information. 
Our architecture is a two-layer GCN~\cite{kipf2017GCN}: 
\begin{equation}
GCN(\hat{\adj},\xmat) = \texttt{ReLU}(\hat{\adj}\cdot\underbrace{\texttt{SeLU}(\hat{\adj}\xmat\wmat^{[0]})}_{\xmat^{[1]}}\wmat^{[1]})
\label{eq:model}
\end{equation}
\textcolor{blue}{where we use $\texttt{SeLU}$~\cite{Klambauer2017activation} and $\texttt{ReLU}(\xvec)=\max(0, \xvec)$ as non-linear activation functions in first and second layer respectively. }

The last layer of our GCN outputs community assignment probabilities through the \texttt{softmax$(\xvec)_i=\frac{e^{\xvec_i}}{\sum_j e^{\xvec_j}}$} activation function. 
\begin{equation*}
\cmat = \texttt{softmax}(GCN(\hat{\adj}, \xmat))
\end{equation*}

This architecture, although simple, allows for propagating information over the entire graph, thus capturing relationships within the graph's structure and the nodes' attributes. 
% \textbf\bigskip
% \textbf{Encoder for soft cluster assignment and node representation} Both encoders of our models are two layers Graph Convolutional Network (GCN) model (Kipf \& Welling)\cite{kipf2017GCN}. 
% The CoDe-GCN encoder is as follows: 

% \begin{equation}\label{eq:Encoder2}
%     GCN (X,A)= \hat{D}^{-1/2}\hat{A}\hat{D}^{-1/2}X\theta
% \end{equation}
% \begin{equation}
%     H_1=\sigma(GCN (X,A))
% \end{equation}
% \begin{equation}
%     \mathcal{E}(X,A)=\sigma(GCN (H_1,A))
% \end{equation}


% where  $GCN$ is defined in equation (\ref{eq:Encoder2}). The activation function of the first layer of soft cluster assignment is ReLU. The activation function of the first layer of node representation is SELU. The activation function for the second layer of both models is ReLU. $\hat{A}=A+I_N$ is the adjacency matrix with self-loops, and $\hat D_{ii}=\sum_{i}\hat A_{ij}$ is the diagonal matrix of 
% $\hat A$. \bigskip
}
% In this section we will present our method, \ourmethod that considers both attributes and structure of the graph for detecting the communities. Our model is inspired by the modularity function.

%\subsection{\ourmethod} 
% We proposed a GNN-based approach that optimizes the modularity in the network by utilizing the contrastive type objective function. We proposed two encoders with the same objective functions. One encoder generates the cluster assignments of the nodes. The other encoder generates node representations for the graph. The proposed contrastive objective function is fully differentiable and optimizes both soft clustering and node representations in an unsupervised manner.


%%% This is NOT our objective - this is our method. 
% our objective is to learn two encoders:

% first, $\mathcal{E}: {\mathbb{R}^{N \times F}} \times {\mathbb{R}^{N \times N}} \overrightarrow{} {\mathbb{R}^{N \times F'}}$ such that $E(X,A)=H=\{\vec{h_1},\vec{h_2},\vec{h_3}...,\vec{h_N}\}$ represents high-level representations $\vec h_i \in \mathcal{R^{F'}}$ for each node $i$. These representations are used for detecting communities in the graph.

% Second, $\mathcal{E}: {\mathbb{R}^{N \times F}} \times {\mathbb{R}^{N \times N}} \overrightarrow{} {\mathbb{R}^{N \times F'}}$ such that $E(X,A)=H=\{\vec{h_1},\vec{h_2},\vec{h_3}...,\vec{h_N}\}$ represents the  associated probability  $\vec h_i \in \mathcal{R^{F'}}$ for each node $i$ to communities. 




\ia{\subsubsection{Contrastive modularity loss}
The GCN loss function is crucial in describing the properties that communities detected by the model will have. As discussed above, a GCN that maximizes only modularity as a single score inherits its limitations, such as a tendency to favor overly small communities. Combining many loss functions, on the other hand, results in a brittle model where parameter tuning quickly becomes an intricate process.

We propose a contrastive loss that mitigates these shortcomings by contrasting node representations from the input graph with those computed on a corrupted graph $\widetilde{\Gr}$, where the latter should not show the same community structure. In this way, the GCN is encouraged to bypass representations that do not convey the community structure in the input graph. On the corrupted graph, the GCN outputs a corrupted assignment $\tilde{\cmat}$.

In the input graph, we define the vector $\mvec$ as 
\begin{equation*}
    \mvec= \Diag\left(\frac{{\cmat^\top}\bmat{\cmat}}{2|\E|}\right)
\end{equation*}
\blue{If we omit the rewiring part, the $\tilde{m}$ formula should be revised}
Analogously for the corrupted graph, we define $\widetilde{\mvec}$ as
\begin{equation*}
    \widetilde{\mvec}=\Diag\left(\frac{\tilde{\cmat}^\top \bmat\tilde{\cmat}}{2|\E|}\right)
\end{equation*}
Intuitively, vector $\mvec$ ($\tilde{\mvec}$, respectively) represents the relative density of each of the communities in the input (corrupted, respectively) graph. 

To compute our objective, we transform community detection into a classification problem in which the model learns how to discriminate real communities from corrupted communities.

Given an indicator variable $\yvec$ such that $\yvec_i = 1$ if $i$ is a community from the input graph, and 0 otherwise, \ourmethod's loss function is
% In order to optimize the cluster assignment matrix the following objective function is proposed. The proposed objective function optimizes modularity through contrastive operation. For optimization,  we use a noise-contrastive type objective with a standard binary cross-entropy (BCE) loss between the samples from the positive examples and negative examples. The proposed objective function is as follows:

\begin{equation}
\mathcal{L}_{\ourmethod}=-\frac{1}{2k}\left( \sum _{i=1}^{k} \yvec_i \log ({\mvec}_i) + \sum _{i=1}^{k} (1-\yvec_{i}) \log (1-\widetilde{\mvec_i})\right)
\label{eq:objective}
\end{equation}
Note that the loss promotes representations for which the modularity is high in the input graph rather than in the corrupted one. Figure~\ref{fig:modularity} demonstrates this difference in the modularity score of a real vs corrupted graph as learning evolves.

Please note that Eq.~\ref{eq:objective} is fully differentiable since it is the composition of differentiable functions, and is therefore amenable to gradient descent optimizers, such as Adam~\cite{kingma2014adam}.
% Where $k$ is the number of communities, $\tilde{k}$ is the number of communities of negative samples. \dm{In our case,} the number of communities in both negative and positive samples is equal. $H$ is the representation of positive samples and $Mod(H)$ is obtained from {refer to equation 9}.  $Mod(\tilde{H})$ is the y is the true class of the modularity of each community. The $y_i$ is 1 for the modularity of the positive samples. $y_i$ is 0 for the modularity of the negative samples.
%\input{figs/fig-modularity}     
}

\subsubsection{Generating the corrupted graph.} \ia{The generation of the corrupted graph $\tilde{\Gr}$ is fundamental to obtaining good node representations. 

A corrupted graph that still remains too similar to the input graph $\Gr$ would not provide the necessary contrast. Technically, it would have a negative impact on the loss in Eq.~\ref{eq:objective} by collapsing the representations of the two graphs. On the other hand, a corrupted graph that bears almost no similarity to the input graph would not carry enough community structure to allow the GCN to capture relevant differences in learning the representations. 


\textcolor{blue}{Should we omit Rewiring part? We can also keep it but we use Andrew's explanation to prove that shuffling is a better choice}

In order to obtain corrupted graphs that exhibit adequate contrast to the input graphs, we propose two strategies. They take outset in graph-theoretical intuitions and the design of our loss function. 

%We introduce two strategies for generating negative samples.

\begin{enumerate}
    \item \textbf{Rewiring}: we rewire the graph such that we still retain the degree of each node $\dg_i$, but choose $\dg_i$ nodes in the graph uniformly without replacement to connect to. Such a rewiring process is theoretically studied in models such as the Watts-Strogatz graph generator~\cite{watts1998collective}.
    \item \textbf{Shuffling}: we permute uniformly at random the vector $\mvec$ in the original graph. This process retains the overall modularity score $Q$, but tends to generate communities with distorted densities, informing the loss function to preserve densities. 
\end{enumerate}
}


\subsubsection{Overview of \ourmethod} 
\ia{Finally, we provide an overview over the major steps in \ourmethod. The algorithm generates  representations through our trainable architecture in Eq.~\ref{eq:model} and the loss function in Eq.~\ref{eq:objective}, to return soft cluster assignments $\cmat$. 
The overall process is the following:

\begin{enumerate}
    \item Compute the soft cluster assignment $\cmat$ for the input graph, training the GCN model in Eq.~\ref{eq:model}.
    \item Compute the soft cluster assignment $\tilde{\cmat}$ for the corrupted graph using the same model as in step (1).
    \item Compute vector $\mvec$ for the input graph, and vector $\tilde{\mvec}$ for the corrupted graph.
    \item Update the parameters of the $GCN$ model via gradient descent to minimize the loss function in Eq.~\ref{eq:objective}.
\end{enumerate}


} 




% Below we give an overview of \ourmethod. In the following setup we give an overview of the steps of soft cluster assignment for each nodes. Moreover, we use the first negative sample generation startegy (generating corrupted graph) 





==> content/old/4.solution.tex <==
%!TEX root=../main.tex
\section{Our solution: \ourmethod}\label{sec:solution}

% \cmt{We need to put a figure with the model's architecture} 


%%%% ANDREW THOUGHTS %%%%
\dmw{
\ia{
\dmk{Our model \ourmethod integrates the simplicity of single-objective community detection with the power of combined scores, by virtue of} a new loss function that encourages \dmk{robust} community memberships while maintaining consistent separation between dissimilar nodes.
}
}

\subsection{\ourmethod Loss function}
\label{ssec:loss}

\dmw{
We build our loss function based on community modularity in Equation~\ref{eq:modularity1}. 
We start out by showing that the entire matrix $\cmat^\top\bmat\cmat$ can be interpreted as the modularity \dmk{\emph{across}} communities. 
Afterward, we introduce our contrastive loss and show how such a loss aims to detect overlapping and non-overlapping communities alike.}

\dmw{
\subsubsection{$\cmat^\top\bmat\cmat$ as modularity across communities.} 
\dmk{We observe that} $\cmat^\top\bmat\cmat$ encodes the modularity matrix at the community scale}
\begin{align*}
    \cmat^\top\bmat\cmat &= \cmat^\top\left(\adj - \frac{\dvec\dvec^\top}{2|\E|}\right)\cmat \\
    &= \underbrace{\cmat^\top\adj\cmat}_{\adj^\Cl} - \frac{1}{2|\E|}\underbrace{(\cmat^\top\dvec)(\dvec^\top\cmat)}_{\dmat_\Cl\dmat_\Cl^\top} =  Q_M
\end{align*}
\dmw{We refer to $Q_M$ as the community-wise modularity matrix.}

\dmw{
If we assume that $\cmat$ is binary, such that $\cmat \in \{0, 1\}^{\nn \times k}$, then $Q_M$ reasonably represents the modularity across the community graph. Note that $\adj^\Cl$ is \dmk{the weighted adjacency matrix of a graph where nodes are communities and the weight $\adj^\Cl_{ij}$ is twice} the number of edges between community $\Cl_i$ and community $\Cl_j$. The diagonal entries $\adj^\Cl_{ii}$ therefore represent the weight from community $i$ to itself and are equal to double the number of edges between the nodes within community $\Cl_i$. \dmk{We also observe} that $\dmat_\Cl = \cmat^\top\dvec$ is the \dmk{community degree matrix and that $\dmat_\Cl \dmat_\Cl^\top / (2|\E|)$ represents the likelihood of an edge existing between communities}. 
%As in the traditional modularity matrix, we scale $\dmat_\Cl \dmat_\Cl^\top$ by $1/2|\E|$, i.e., the total sum of elements in $\adj^\Cl$. 
As such, we can interpret $Q_M$ as the modularity of the graph in \dmk{which nodes} are replaced with their corresponding communities.}

\dmw{
In the more practical case of non-binary community memberships with $\cmat \in [0,1]^{\nn \times k}$, we can interpret $Q_M$ as the modularity across ``fuzzy'' communities, where each entry of the matrix is proportional to the corresponding community membership strengths.
}

\dmw{
Given this analysis, with \dmk{$\cmat$ representing probabilities} that nodes belong to different communities, we devise the loss function
}
\begin{equation}
\mathcal{L}_{\ourmethod}=-\frac{1}{2k}\sum_{i=1}^{k} \left( \log (\Diag(\sigma(Q_M))_i) + \log (1- \Diag(\mathcal{P}(\sigma(Q_M)))_i)\right)
\label{eq:objective}
\end{equation}
\dmw{where $\Diag$ \dmk{extracts the vector of the diagonal of a matrix}, $\mathcal{P}$ returns a random row-permuted matrix, and $\sigma$ is the sigmoid function. The row permutation ensures that every community is compared repulsively to its counterparts, as the post-permutation diagonal contains the community modularity between separate communities.}
\dmw{
Our loss function in Eq.~\ref{eq:objective} \dmk{maximizes} the diagonal elements of $Q_M$, i.e., the modularity within a community, and minimizes the off-diagonal elements, i.e., the modularity across communities. This loss function thus has the straightforward interpretation of clustering similar groups of nodes while encouraging separation between dissimilar ones.

Note that $\mathcal{L}_{\ourmethod}$ has a natural analog to cross-entropy and contrastive objective functions. We can consider a target distribution $\yvec \in \{0, 1\}^{2k}$, where $\yvec_i$ is 1 when observing diagonal elements of $Q_M$ (the first $k$ elements of $\yvec$) and $0$ when observing off-diagonal elements (the last $k$ elements), giving us}

\begin{align*} 
\mathcal{L}_{\ourmethod}=-\frac{1}{2k}\sum_{i=1}^{k} & \left(( \yvec_i \log (\Diag(\sigma(Q_M))_i) +\right. \\
                                                                    & \left. (1 - \yvec_{k+i})\log (1- \Diag(\mathcal{P}(\sigma(Q_M)))_i) \right)
\end{align*}
\dmw{Thus, $\mathcal{L}_{\ourmethod}$ can be viewed through the lens of general contrastive learning, where the positive samples compare a community with itself and negative samples compare separate communities. In this interpretation, our similarity measure is the community-wise modularity of the samples.
}



\subsubsection{A loss for overlapping and non-overlapping communities}
\dmw{
\dmk{Can our loss capture both overlapping and non-overlapping communities, without penalizing any of the two formulations?} First note that Eq.~\ref{eq:objective} is not dependent on whether the communities are overlapping. We define overlap as the cosine similarity between the columns $\cvec_{i}$ of $\cmat$ that represent community indicator vectors. We define a multi-objective minimization problem
}
\begin{align*}
    f_1(\cvec_i, \cvec_j) &= \underbrace{\cvec_i^\top\adj\cvec_j + \frac{1}{2|\E|} (\cvec_i^\top \dvec) (\dvec^\top\cvec_j) }_{\mathcal{L}_{\ourmethod} \text{ for communities }i,j} \\
     f_2(\cvec_i, \cvec_j) &= \left( \frac{\cvec_i^\top \cvec_j}{\|\cvec_i\| \|\cvec_j\|} \right)^2
\end{align*}
\dmw{
If our loss function required either overlapping or non-overlapping communities, then the above multi-objective optimization problem would have a Pareto optimal solution. Clearly, $f_2$ is minimized when the vectors are orthogonal. \dmk{Please note that minimizing $f_1$ does not necessarily lead to the minimization of $f_2$, which would mean that our objective only encourages non-overlapping communities. On the contrary, we} can see that, by computing the partial derivative of $f_1$ with respect to $\cvec_i$
} we obtain
\[ \nabla_{\cvec_i} f_1 = \cvec_j^\top \adj^\top + \frac{1}{2|\E|} \dvec \cvec_j^\top\dvec^\top\]
\dmw{
Now we can see that if $\cvec_i$ and $\cvec_j$ are orthogonal, the gradient is not necessarily $0$ and instead depends on the interaction of the remaining indicator vector with the graph. As such, our objective function does not require orthogonal communities and can simultaneously be used for overlapping and non-overlapping community detection. We support this intuitive explanation with compelling empirical results on non-overlapping and overlapping community detection alike (Section \ref{sec:experiments}).
}


\ia{\subsection{\ourmethod architecture} 

\dmw{The main purpose of our GCN is to learn the community assignment matrix $\cmat$ using \dmw{the graph structure and the node attributes.} 
Our architecture is a two-layer GCN~\cite{kipf2017GCN}: }
\begin{equation}
GCN(\hat{\adj},\xmat) = \texttt{ReLU}(\hat{\adj}\cdot\underbrace{\texttt{SeLU}(\hat{\adj}\xmat\wmat^{[0]})}_{\xmat^{[1]}}\wmat^{[1]})
\label{eq:model}
\end{equation}

\dmw{The last layer of our GCN outputs community assignment probabilities via the function \texttt{Norm$(\xvec)_i=\frac{\xvec_i}{\sum_j \xvec_j}$}. }
\begin{equation*}
\cmat = \texttt{Norm}(GCN(\hat{\adj}, \xmat))
\end{equation*}

\dmw{This architecture, although simple, allows for propagating information over the entire graph, thus capturing relationships within the graph's structure and the nodes' attributes. }}

\subsubsection{Adapting to regularization}\label{solution:log}
We note that the values in $Q_M$ can be positive or negative and are not necessarily bounded. The sigmoid is thus necessary in order to calculate the cross-entropy to the target distribution. However, we found empirically that the division by $4|\mathcal{E}|$ in Eq. \ref{eq:mod_matrix} settles the values in $\cmat^\top\bmat\cmat$ close to 0, leaving the sigmoid outputs near $1/2$. This does not present an issue in lightly-regularized learning environments but may hamper learning when applying sufficient regularization. In order to overcome this, we propose amplifying the values in $\cmat^\top\bmat\cmat$ by applying a logarithm to the $\cmat$ matrix after the $\texttt{Norm}$. In preliminary experiments, we empirically confirmed that this approach sufficiently amplifies the values so as to achieve good performance when using network regularization.


%\aad{
%We also investigate $L_{\ourmethod}$'s effect on community sizes. We can define the diagonal elements by $Q_{M}^{ii} = c_i^TAc_i - 1/(2|\mathcal{E}|) c_i^Tdd^Tc_i$. Then optimizing $L_{\ourmethod}$ involves:
%\begin{enumerate}
    %\item maximizing $c_i^TAc_i$; this occurs when $c_i$ captures a part of the graph with many edges
    %\item minimizing $1/(2|\mathcal{E}|) c_i^Tdd^Tc_i$; this occurs when the sum of degrees of nodes in $c_i$ goes to zero
%\end{enumerate}
%This limit-case analysis implies that $L_{\ourmethod}$ encourages communities to neither be too small nor too large. \cmt{should we take this part out?}
%}

%%%% ANDREW THOUGHTS %%%%


% \subsubsection{Generating the corrupted graph.} \cmt{We don't really have a corrupted graph anymore} \ia{The generation of the corrupted graph $\tilde{\Gr}$ is fundamental to obtaining good node representations. 

% A corrupted graph that still remains too similar to the input graph $\Gr$ would not provide the necessary contrast. Technically, it would have a negative impact on the loss in Eq.~\ref{eq:objective} by collapsing the representations of the two graphs. On the other hand, a corrupted graph that bears almost no similarity to the input graph would not carry enough community structure to allow the GCN to capture relevant differences in learning the representations. 


% \textcolor{blue}{Should we omit Rewiring part? We can also keep it but we use Andrew's explanation to prove that shuffling is a better choice}

% In order to obtain corrupted graphs that exhibit adequate contrast to the input graphs, we propose two strategies. They take outset in graph-theoretical intuitions and the design of our loss function. 

% %We introduce two strategies for generating negative samples.

% \begin{enumerate}
%     \item \textbf{Rewiring}: we rewire the graph such that we still retain the degree of each node $\dg_i$, but choose $\dg_i$ nodes in the graph uniformly without replacement to connect to. Such a rewiring process is theoretically studied in models such as the Watts-Strogatz graph generator~\cite{watts1998collective}.
%     \item \textbf{Shuffling}: we permute uniformly at random the vector $\mvec$ in the original graph. This process retains the overall modularity score $Q$, but tends to generate communities with distorted densities, informing the loss function to preserve densities. 
% \end{enumerate}
% }


% \subsubsection{Overview of \ourmethod} 
% \ia{Finally, we provide an overview over the major steps in \ourmethod. The algorithm generates  representations through our trainable architecture in Eq.~\ref{eq:model} and the loss function in Eq.~\ref{eq:objective}, to return soft cluster assignments $\cmat$. 
% The overall process is the following:

% \begin{enumerate}
%     \item Compute the soft cluster assignment $\cmat$ for the input graph, training the GCN model in Eq.~\ref{eq:model}.
%     \item Compute the soft cluster assignment $\tilde{\cmat}$ for the corrupted graph using the same model as in step (1).
%     \item Compute vector $\mvec$ for the input graph, and vector $\tilde{\mvec}$ for the corrupted graph. \cmt{We do not really have a corrupted graph anymore}
%     \item Update the parameters of the $GCN$ model via gradient descent to minimize the loss function in Eq.~\ref{eq:objective}.
% \end{enumerate}


%}




% Below we give an overview of \ourmethod. In the following setup we give an overview of the steps of soft cluster assignment for each nodes. Moreover, we use the first negative sample generation startegy (generating corrupted graph) 





==> content/old/5.experiments.tex <==
%!TEX root=../main.tex

\section{Experiments}\label{sec:experiments}

% This can be moved in the appendix, if necessary.

%The code is available at \cmt{anon url?}. \cmt{describe libraries.}} 
%Check the section of overlapping later

\amw{\dmw{In this section, we compare \ourmethod with state-of-the-art approaches for community detection on several benchmark graph datasets. We analyze in Section~\ref{ssec:nonoverlapping} our results in both non-overlapping community detection (graph partitioning) and overlapping community detection where nodes may be assigned to more than one community (Section~\ref{ssec:overlapping}). We further analyse the sensitivity of our approach to its few hyperparameters (Section~\ref{ssec:tuning}). 
}%Our results show that our method returns more significant communities than single score methods while requiring no post-processing of the features with kmeans or othe clustering algorithms.
}   

\input{figs/fig-nmi-nonoverlapping}
\input{figs/fig-f1-nonoverlapping}



\subsection{Non-Overlapping Community Detection}\label{ssec:nonoverlapping}

\dm{\para{Datasets.} 
\dmw{We perform our experiments on seven real-world networks.}
\cora, \citse, and \pubmed~\cite{sen2008collective} are co-citation networks among papers where attributes are bag-of-words representations of the paper's abstracts, and labels are paper topics. 
\dmk{\amzph and \amzpc ~\cite{shchur2018pitfalls}  are subsets of the Amazon co-purchase graph with the frequency of products purchased together; attributes are bag-of-words representations of product reviews, and class labels are product categories.
\coacs and \coaphy~\cite{shchur2018pitfalls} are co-authorship networks based on the MS Academic
Graph for the computer science and physics fields respectively;  attributes are collections of paper keywords; class labels indicate common fields of study.}
\dmk{Our choice of datasets include graphs with different densities and characteristics, as well as the largest networks evaluated by the competitors.}
% These datasets were chosen due to the availability of ground-truth labels and ease of access. Note that neither we nor our competitors evaluate on datasets with $100K+$ nodes as these do not have ground-truth information readily available.}
\dmk{The characteristics of the datasets are summarized in Table~\ref{tbl:datasets}.}}


\input{tables/tbl-datasets}

\ia{\para{Competitors.} We evaluate our method against the following established state-of-the-art methods: 
\begin{itemize}[leftmargin=*]
\item \textbf{kmeans (features)} clusters node attributes with the kmeans++ algorithm~\cite{David2007kmeans}. It provides an indication of the importance of attributes for community detection, where it is often used in connection with the clustering of node embeddings.
\item\textbf{DGI+kmeans}: Deep Graph Infomax (DGI)~\cite{velivckovic2018deep} is an unsupervised GNN model that attains competitive performance on node classification, link prediction, and graph classification. As DGI is not a community detection GNN, we first obtain the DGI node representations and then run kmeans on these representations. 
\item\textbf{MinCut}~\cite{bianchi2020spectral} is a graph pooling technique that trains a GNN using a min-cut loss similar to spectral clustering~\cite{shi2000normalized} for community detection; MinCut generates soft cluster assignments. 
\item\textbf{DMoN}~\cite{tsitsulin2020graph} is a state-of-the-art community detection model that trains a shallow GCN with the explicit goal of optimizing the graph modularity. 
\dmk{\item\textbf{NOCD}~\cite{shchur2019overlapping} is the state-of-the-art GNN for overlapping community detection. We assign each node to the cluster with the highest probability.} 
\end{itemize}}



\input{tables/tbl-ucode-kmeans}


\input{tables/tbl-conductance-nonoverlapping}


\dm{\spara{Our methods.} We study two different versions of our algorithm for \dmw{detecting overlapping communities.}
The first, \dmw{\ourmethod, outputs soft community predictions as an assignment matrix $\cmat$ that assigns a probability $p_{ij}$ that node $v_i$ belongs to community $j$. For non-overlapping community detection, we assign the node to the community with the highest probability, i.e., $\max_j p_{ij}$.}

The second, \ourmethod{+}kmeans \dmk{applies the kmeans algorithm on the representations obtained by the ReLU function} in Eq.~\ref{eq:model}. Through this extension, we aim to show the validity of our method against decoupled community detection approaches.} 

\dmk{The first analysis in Figure~\ref{tbl:ucode-kmeans} reports the results comparing these two versions of \ourmethod. The results suggest that kmeans contributes only marginal quality improvement, which confirms the validity of our efficient end-to-end loss function for community detection.}

\dm{\spara{Quality measures.} We report the average results of four measures to \dmw{qualify different, but related aspects of the detected communities.}

We first compare with ground-truth communities and report the Normalized Mutual Information (NMI) and pairwise F1 score between nodes and communities, which indicate how well the detected communities match the ground-truth communities. \dmk{In the interest of readability, we multiply all result values by $100$.}}

We also include two intrinsic graph measures. \dmk{The cluster conductance ($\mathcal{C})$~\cite{Yang2015conductance} 
%is heavily influenced by the application of graphs to electrical circuits. It 
measures how well-connected the nodes in the communities are related to the escape probabilities of random walks. Modularity($Q$)~\cite{newman2006modularity} assesses whether intra-community nodes are more densely connected than their inter-community counterparts. \dmk{In order to address the modularity's tendency to prefer smaller communities, we perform experiments that span over the ground-truth communities and inspect the effect that number of communities have on our results. For this reason, the number of communities in the datasets used in our evaluation range from $3$ to $43$.}}

\dm{\spara{Parameter settings.}
We repeat each experiment $10$ times, train the model for $500$ epochs, and report the average result among the runs.
\ourmethod GCN has two layers with $512$ dimensions. The number of communities $k$ \ourmethod produces is $k=16$ for all datasets. \dmk{
$k=16$ is also the default choice for MinCut~\cite{bianchi2020spectral} and DMoN~\cite{tsitsulin2020graph}. In preliminary experiments, we also evaluated different values of $k = 8, k=32$ but consistently found inferior results. As such, also for a fair comparison with the previous models, we set $k=16$. }
\ourmethod{+}kmeans has an output layer with $512$ dimensions. 
Both models use a dropout between [0.1, 0.3]. We use dropout 0.1 on all datasets except for \pubmed in which we use dropout 0.3. We apply batch normalization in both internal layers \dmk{and set a learning rate $0.001$ for the Adam optimizer~\cite{kingma2014adam} for learning.} 
\dmw{As propagation layer for our model we additionally } performed preliminary experiments with GraphSAGE~\cite{hamilton2017inductive} but opt for GCNs~\cite{kipf2017GCN} due to their superior performance in our analyses. 
%We also experimented our model using GraphSAGE~\cite{Hamilton2017Graphsage} convolutional and the results were inferior to the GCN~\cite{kipf2017GCN}. 
}

\subsubsection{Community detection results}\label{sssec:nonoverlapping}
% \cmt{Davide: To Revise}





\dmk{We begin our experimental evaluation with an overall comparison of methods for non-overlapping community detection across different datasets. As Figure~\ref{fig:nmi-nonoverlapping} confirms, \ourmethod is the most robust choice for non-overlapping communities in all seven datasets. Regardless of dataset characteristics, we observe that \ourmethod obtains competitive results, where existing approaches fail to perform on at least some of the datasets. Indeed, a more detailed analysis reveals that \ourmethod ranks \textit{on average} higher than any other competitor. Figure~\ref{fig:f1-nonoverlapping} confirms the same behaviour on F1 score. 

We note also that on the denser \amzpc and \amzph methods like MinCut fail to converge. They also provide overall lower scores, indicating that graph pooling cannot be a viable approach for the community detection task. Our method clearly outperforms traditional methods, such as kmeans, demonstrating an advantage of a graph-learning approach over attribute clustering to capture the structural characteristics of a graph. Finally, DGI+kmeans generally produces unsatisfactory results, yet requires a separate clustering of embeddings. NOCD fares relatively good against methods explicitly targeting non-overlapping communities, but still fails to provide competitive results against \ourmethod. 

We now turn our attention in Figure~\ref{tbl:C-Q-nonoverlapping} to conductance ($\mathcal{C}$) and modularity ($Q$). \ourmethod shows the best performance in terms of conductance, which means that \ourmethod is particularly good at identifying well-connected communities. This makes sense, as our loss function specifically encourages high intra-connections and low inter-connections. At the same time, DMoN, which optimizes for modularity, does not consistently attain the best modularity, indicating the hardness of the objective.  However, our method's indirect modularity optimization obtains comparable modularity on \coaphy and even outperforms DMoN on \cora and \amzph. This indicates that the contrastive loss in \ourmethod indeed yields more nuanced community structure than can be obtained through optimizing modularity alone. This is even more notable when considering the other measures where \ourmethod outperforms DMoN. }

\dmk{In conclusion, the empirical evaluation clearly shows that our model is highly robust and widely applicably, obtaining competitive results across the evaluation metrics and datasets rather than targeting any single one. While methods that directly optimize traditional modularity will achieve good modularity scores, this will be at the expense of performance on other measures. \ourmethod instead achieves competitive results across every metric with little-to-no hyperparameter tuning.}




% On Amazon Photo, MinCutPool fails to converge. It produces lower scores overall, indicating that a graph pooling method that optimizes a single objective is not sufficient for capturing all relevant information for community detection in \dmw{attributed graphs.} 


% Moved here as it seemed out of context. 






% \ourmethod produces consistently high-quality results across all four data sets with respect to all four measures. In particular, \ourmethod obtains the best performance with respect to all metrics on Cora and Amazon Photo. 


% \dmk{In all but one case, \ourmethod outperforms the kmeans (features) baseline, often by a large margin. This demonstrates that clustering based on node attributes alone is not sufficient, as it fails to incorporate the structural information in the network. The only exception is the NMI measure on the Pubmed dataset, which is a metric that gives higher importance to producing many small communities than the other measures.}

% DGI+kmeans, which clusters GNN representations using k-means, fairs comparatively poorly with respect to the conductance and modularity measures, indicating that the approach taken in \ourmethod of optimizing directly for community relationships results in communities that are more intraconnected and separated than those obtained when generating representations and clustering afterwards. It obtains slightly higher scores with respect to the NMI and F1 metrics, which account for the identification of nodes alone. On Amazon Photo, however, \ourmethod outperforms DGI+kmeans by a large margin. We expect that this is due to the dataset's higher network density.

% DMoN, which optimizes for modularity alone, obtains the best modularity score on the Pubmed graph. However, our method's indirect modularity optimization obtains comparable modularity on Pubmed and even outperforms DMoN on Cora and Amazon Photo. This implies that the contrastive loss in \ourmethod's loss function indeed yields more nuanced community structure than can be obtained through improving modularity alone. This is even more notable when considering the other measures where \ourmethod outperforms DMoN. 



% Across all datasets, \ourmethod shows the best performance in terms of conductance, which means that \ourmethod is particularly good at identifying well-connected communities. This makes sense, as our loss function specifically encourages high intra-connections and low inter-connections. At the same time, modularity is consistently among the best result values, indicating that \ourmethod successfully finds correct separations between communities and manages to preserve the modularity characteristics. 
% \label{tbl:nonoverlapping}








\subsection{Overlapping community detection} 
\label{ssec:overlapping}
\dmw{Here we} evaluate \ourmethod's performance against overlapping community detection approaches. For \ourmethod, we use the same general model in the overlapping setting, but \dmw{tune the hyperparameters of our model to better reflect overlapping communities. The parameter setting is explained next.}

\spara{Competitors.} We compare \ourmethod against the following baselines and state-of-the-art methods for overlapping community detection:

\begin{itemize}[leftmargin=*]
\dmw{\item\textbf{NOCD}~\cite{shchur2019overlapping} is a GCN that finds overlapping communities by maximizing a Bernoulli-Poisson model likelihood using gradient descent.}
\item\textbf{DMoN}~\cite{tsitsulin2020graph} is a state-of-the-art \dmk{non-overlapping community detection GCN} that generates soft cluster assignments. \dmk{It maximizes modularity which is not inherently tied} to disjoint clusters, allowing us \dmk{to employ it} for detecting overlapping communities. 
\end{itemize}

\dmw{\spara{Quality measures.} We evaluate overlapping community detection on the traditional Facebook~\cite{Jure2014ego-network} datasets (Table~\ref{tbl:datasets}) which is a collection of ego-networks with ground-truth communities, and a much larger dataset \eng~\cite{shchur2019overlapping}. We report the overlapping normalized information (NMI)~\cite{McDaid2011NormalizedMI} 
% This part is copied from bigclam paper
and the recall to assess the model's ability to identify correct cluster memberships. 
We used recall as defined in~\cite{yang2013overlapping}, that is the average recall for best-matching detected communities. Let $\cmat^{*}$ the ground-truth community assignment matrix and $\cmat$ the set of detected communities: 
\begin{equation*}
    Recall(\cmat^{*}, \cmat)=\frac{1}{\cmat^{*}}\sum_{\cvec_{i}\in \cmat^{*}}Rc(\cvec_{i},\cvec{}_{g(i)})
\end{equation*}
}
\dmw{Each ground-truth community $\cvec_{i}\in\cmat^{*}$ and each detected community $\cvec_{j}\in\cmat{}$ is defined by its set of member nodes.  $Rc(\cvec_{i},\cvec_{j})$ is the recall of community $\Cl_{j}$ under the best matching $g$, i.e., the matching with the largest number of nodes from community $i$.}
 
\dmw{\spara{Assigning nodes to communities.} In order to compare the obtained communities to the ground-truth community membership, we convert the predicted soft assignments to binary community assignments. We assign each node to a community if its predicted membership value exceeds a chosen threshold $p$. 
%However, finding the threshold that performs best in all datasets is challenging.
We analyze two different thresholding techniques that perform well on average for all the datasets: $p_{1}=0.5$ and $p_{2}= \mathbb{E}[\cmat|\cmat > 0]$, that is the expected value of the positive assignments. \dmk{These thresholds show similar results in all datasets. We additionally identify that our thresholding techniques correspond to elbow points in a grid search, thus corroborating the threshold validity.} We report the best performance for each dataset between the two thresholds, with \fb-348 and \fb-1912 metrics performing better with the $p_{1}$ threshold while the rest of the datasets use thresholding approach $p_{2}$.
For the NOCD model, we set $p_{1}=0.5$ as in their experiments. We evaluate the DMoN model using both $p_{1}$ and $p_{2}$, but report the $p_2$ results as they were the highest in every experiment. } 


\input{tables/tbl-overlapping-gcn}
%\input{figs/fig-tuning}
\input{figs/fig-ucode-learning}

\input{figs/fig-modularity-epochs}
% \input{figs/fig-modularity}

\dmw{
\spara{Parameter Settings.} The overlapping model has the 2-layer graph convolutional architecture as the corresponding non-overlapping model. We set the size of the first layer to $128$ while keeping the second, and output, layer's size the number of communities $k$. We
apply batch normalization after the first graph convolutional layer with dropout at $0.5$ before every layer. The learning rate is set to $ 10^{-3}$. We add weight decay to both weight matrices with regularization strength $\lambda = 10^{-2}$. Unlike our non-overlapping model, we apply a ReLU in the first layer while Softmax is not applied in the last layer, to allow for smoother soft memberships. We repeat each experiment $10$ times, train the model for $1000$ epochs, and report the average result among the runs.}
% \input{figs/prox-high-school.tex}

\dmw{\subsubsection{Overlapping community detection results} 
We provide results for two forms of each algorithm among NOCD, \ourmethod and DMoN in Table~\ref{tbl:overlapping-gcn1} and Table~\ref{tbl:overlapping-gcn2}. The input of the GCN in \dmk{[model\_name]-X} is node attributes; the input of \dmk{[model\_name]-G} is the concatenation of adjacency and node attributes. As we can see in Table~\ref{tbl:overlapping-gcn1} and  Table~\ref{tbl:overlapping-gcn2}, \ourmethod shows very promising results for overlapping community detection. \ourmethod is the best method overall of the datasets in terms of recall and returns comparably good results on all datasets in terms of NMI. In particular, we note that \ourmethod is consistently better than the corresponding DMoN-X or DMoN-G in nearly all datasets, vindicating our model's choice and validating the claim that our model can competitively detect overlapping and non-overlapping communities. 
This shows that our general community detection model competes with NOCD, which is the only GCN that explicitly optimizes for overlapping community detection.} 


\subsection{Tuning \ourmethod}
\label{ssec:tuning}

\dm{
We analyse \ourmethod as a function of the number of training iterations (epochs) and the embedding dimension of the internal layers. 
\dmw{Figure~\ref{fig:tuning} analyzes non-overlapping community detection.} As expected, the loss decreases with more epochs and stops improving after 100 epochs. 
This behaviour is confirmed in the NMI score. 

We also report the impact of the embedding dimension on NMI. We note that increasing the dimension is beneficial until the dimension reaches 256-512. After that point, the quality plateaus and gently decreases. 
We set the embedding dimension to $512$ in our experiments as it shows more consistent behavior across datasets. We repeat the same analysis of \ourmethod for overlapping community detection \dmw{and observe a similar behavior.} \dmk{The only difference to the non-overlapping model is an even more stable behaviour around $128$ dimensions. In general, a lower embedding dimension is preferable for efficiency and compactness. }}

\dmw{Figure~\ref{fig:modularity-epochs} compares the modularity score for DMoN and \ourmethod\ \dmk{per training epoch.} Our contrastive loss expectedly fluctuates slightly more but finally settles on a higher modularity, which confirms our analysis in Section~\ref{ssec:loss}.}

%\input{figs/exp_basealign.tex}




% \subsection{Comparison to previous methods}

% The main experiment




% \input{figs/time-precomputation.tex}
% \input{figs/time-noprecomputation.tex}


==> content/old/6.conclusions.tex <==
%!TEX root=../main.tex
\section{Conclusion}\label{sec:conclusion}

\ia{We propose \ourmethod, a new Graph Neural Network method for community detection in attributed graphs. \dmw{\ourmethod performs both overlapping and non-overlapping community detection, by virtue of a novel contrastive loss that maximizes a soft version of network modularity. We provide intuitive theoretical justification for our choices and validate our claims on a large set of experiments. Our experimental assessment confirms that our method is expressive and overall superior in both overlapping and non-overlapping community detection tasks, exhibiting competitive performance in comparison with state-of-the-art methods designed for either one of the tasks.} 
%optimizes a novel contrastive loss function that retains the simplicity of single score methods and the effectiveness of combined scores. 
%We devise a novel strategy for generating distorted graphs that provides the desired contrast. In a thorough experimental evaluation, we show that our method attains state-of-the-art performance on a number of datasets, while being easy to tune. In addition, we show that our method can also successfully be used for overlapping community detection. %The introduce a method for both overlapping and non overlapping community detection method is an interesting future direction of this work. %IRA: seems too vague to me, and just to say "we did not get around to it"
}



==> content/old/Revision.tex <==
\appendix

%\section{Revision}\label{sec:revision}
%The loss Function that is in the deep graph infomax paper:


\begin{comment}

\begin{equation}
\mathcal{L}_{DGI}=\frac{1}{N+M}\left( \sum _{i=1}^{N} E(X,A) [\log D( {\vec{h_i}, \vec{s}})] + \sum _{j=1}^{M} E(\tilde{X},\tilde{A}) [\log (1-D({\tilde{\vec{h_j}}, \tilde{\vec{s}}}))]\right)
\label{eq:objective}
\end{equation}
    where N is the number of positive samples, and M is the negative samples. $\tilde{X}$ and $\tilde{A}$ are the features and adjacency matrix of the corrupted graph(negative samples). $\vec{h_i}$ is the node representations of the original graph, and $\vec{s}$ is the summary vector of the original graph, and $h_j$ is the node representations of the corrupted graph. The $\mathcal{D}$ is a bilinear scoring function:
    \begin{equation}
                \mathcal{D}(\vec{h_i},\vec{s})=\sigma({\vec{h_i}^{T}}W{\vec{s}})
    \end{equation}
    The following equation represents how we obtain the summary vector. 
    \begin{equation}
        \vec{s}= \frac{1}{N}\sum_{i=1}^{N}{\vec{h_i}}
    \end{equation}
    
      Where $\sigma$ is the logistic function, and W is the learnable weight matrix.
      The function mentioned above is based on the Jensen-Shannon Divergence method. The objective of this method is to measure the similarity between two distributions which maximizes the mutual information between the summary vector and the node representations.

\textbf{The idea behind this loss function is that the above loss function maximizes the mutual information between $\vec{{h_i}}$ and $\vec{s}$, based on the Jensen-Shannon divergence between the positive and the negative samples.}


\textbf{Can we consider bilinear scoring function as a probability?}

Overview of Deep Graph infomax from their code ?

Generate a lbl vector: $lbl=(1,1,1,..,0,0,0,..)$

\bigskip

Then the $logits$ will be extracted. The $logits$ are the output of bilinear function in each iteration.

$logits=(Positive-samples , Negative-samples )$

The loss function would be as follows:

\begin{equation}
\mathcal{L}_{DGI}(logits,lbl)=-w_{n}[(lbl_n \log \sigma(logits_n) + (1-lbl_n) \log (1-\sigma(logits_n))]
\label{eq:objective}
\end{equation}
\textbf{They actually minimize the above loss function.}


The loss function that we currently have :

\begin{equation}
\mathcal{L}_{CoCoDe}=-\frac{1}{2k}\left( \sum _{i=1}^{k} \yvec_i \log (\widetilde{\mvec}_i) + \sum _{i=1}^{k} (1-\yvec_{i}) \log (1-\mvec_i)\right)
\label{eq:objective}
\end{equation}

I made a mistake , the positive and negative samples should be reverse.

\begin{equation}
\mathcal{L}_{CoCoDe}=-\frac{1}{2k}\left( \sum _{i=1}^{k} \yvec_i \log (\mvec_i) + \sum _{i=1}^{k} (1-\yvec_{i}) \log (1-\widetilde{\mvec_i})\right)
\label{eq:objective}
\end{equation}

Can we rewrite it like Deepgraph infomax?

\begin{equation}
\mathcal{L}_{CoCoDe}=\frac{1}{N+M}\left( \sum _{i=1}^{N} E(C,B) \log (\mvec_i) + \sum _{j=1}^{M} E(\tilde{C},\tilde{B}) [\log (1-\widetilde{\mvec_i})\right)
\label{eq:objective}
\end{equation}
\end{comment}





%\input{figs/fig-modularity-DMoN}



==> examples/alg-grasp.tex <==
\begin{algorithm}[!h]
\begin{algorithmic}[1]
% \small
\Require{Graphs $G_1 = (V_1, E_1)$, $G_2 = (V_2, E_2)$}
\Params{Eigenvectors $k$, corresponding functions $q$, time steps $t=[t_1,\ldots,t_q]$}
%\Ensure{An action $(v, \fidelity)$}
\smallComment{Step 1: Eigendecomposition of Laplacian}
\State $\lapl_1\gets\eye-D_1^{-\frac{1}{2}}A_1D_1^{-\frac{1}{2}}$, $\lapl_2\gets\eye-D_2^{-\frac{1}{2}}A_2D_2^{-\frac{1}{2}}$
% \smallComment{Step 2: Eigendecomposition of Laplacians}
\State $\Phi,\Lambda_1 \gets \eig(\lapl_1)$
\State $\Psi,\Lambda_2 \gets \eig(\lapl_2)$
\smallComment{Step 2: Compute corresponding functions}
\ForAll{$t_i$ in $t$} 
\State $f_i\gets \sum_{j=1}^n e^{-{t_i}\lambda_j}\phi_j \odot \phi_j$
\State $g_i\gets \sum_{j=1}^n e^{-{t_i}\lambda_j}\psi_j \odot \psi_j$
\EndFor
\State $F \gets [f_1, \ldots, f_q]$
\State $G \gets [g_1, \ldots, g_q]$
\smallComment{Step 3: Base alignment}
\State $\bar{\Phi}=[\phi_1,\ldots,\phi_k]$
\State $\bar{\Psi}=[\psi_1,\ldots,\psi_k]$
\State $M\gets\min_{M\in S(k,k)}\off(M^\top\bar{\Lambda}_2 M)+\mu\|F^\top\bar{\Phi}-G\bar{\Psi} M\|_F^2$
\State $\hat{\Psi}=\bar{\Psi}M$
\smallComment{Step 4: Calculate mapping matrix}
\State\begin{equation*}
\min_{[c_{11},\ldots,c_{kk}]^\top}\left\Vert\begin{bmatrix}
    \diag(g_1^\top\hat{\Psi})\\
    \vdots\\
    \diag(g_q^\top\hat{\Psi})
\end{bmatrix}
    \begin{bmatrix}
    c_{11}\\
    \vdots\\
    c_{kk}
\end{bmatrix}
-  \begin{bmatrix}
    \bar{\Phi}^\top f_1\\
    \vdots\\
    \bar{\Phi}^\top f_q
\end{bmatrix}
\right\Vert_2^2
\end{equation*}
\State $C\gets\diag([c_{11},\ldots,c_{kk}]^\top)$
%\smallComment{align eigenvectors with C}
\smallComment{Step 5: Matching by linear assignment}
\State $N\gets$ Matching of columns of $\bar{\Phi}^\top$ to those of $C\hat{\Psi}^\top$ 
\State\Return $N$
\end{algorithmic}
\caption{\thiswork}\label{alg:grasp}
\end{algorithm}

==> examples/exp_accuracy.tex <==
\begin{figure*}
\centering
\begin{subfigure}{.32\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{figs/arenas_accs_hun.png}  
  \caption{Arenas}
  \label{fig:quality:others_arenas}
\end{subfigure}
\begin{subfigure}{.32\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{figs/facebook_accs_hun.png} 
  \caption{Facebook}
  \label{fig:quality:others_facebook}
\end{subfigure}
\begin{subfigure}{.32\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{figs/CA-AstroPh_accs_hun.png} 
  \caption{CA-AstroPh}
  \label{fig:quality:others_CA-AstroPh}
\end{subfigure}
\vspace{-3mm}
\caption{Accuracy compared to REGAL~\protect\cite{heimann18regal} and Low Rank EigenAlign~\protect\cite{nassar2018lowrank}}
\label{fig:quality}
\vspace{-3mm}
\end{figure*}




% \begin{figure*}
% \centering
% \begin{subfigure}{.32\textwidth}
%   \centering
%   \includegraphics[width=1\linewidth]{figs/time_precomputed.png}  
%   \caption{Precomputed}
%   \label{fig:others_arenas}
% \end{subfigure}
% \begin{subfigure}{.32\textwidth}
%   \centering
%   \includegraphics[width=1\linewidth]{figs/time_precomputed.png} 
%   \caption{Not precomputed}
%   \label{fig:others_facebook}
% \end{subfigure}
% \vspace{-3mm}
% \caption{Computation times of GASP and its closest competitor REGAL}\label{fig:time}
% \vspace{-3mm}
% \end{figure*}

==> examples/exp_basealign.tex <==
% \begin{figure*}
% \centering
% \begin{subfigure}{.32\textwidth}
%   \centering
%   \includegraphics[width=1\linewidth]{figs/arenas_others_accs_nn_hun.png}  
%   \caption{Arenas}
%   \label{fig:others_arenas}
% \end{subfigure}
% \begin{subfigure}{.32\textwidth}
%   \centering
%   \includegraphics[width=1\linewidth]{figs/facebook_others_accs_nn_hun.png} 
%   \caption{Facebook}
%   \label{fig:others_facebook}
% \end{subfigure}
% \begin{subfigure}{.32\textwidth}
%   \centering
%   \includegraphics[width=1\linewidth]{figs/CA-AstroPh_others_accs_nn_hun.png} 
%   \caption{CA-AstroPh}
%   \label{fig:others_CA-AstroPh}
% \end{subfigure}
% \vspace{-3mm}
% \caption{Accuracy compared to REGAL~\protect\cite{heimann18regal} with nearest neighbor alignment and jv alignment}\label{fig:parameters}
% \vspace{-3mm}
% \end{figure*}


\begin{figure*}
\centering
\begin{subfigure}{.32\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{figs/variants_arenas.png}  
  \caption{Arenas}
  \label{fig:variants:others_arenas}
\end{subfigure}
\begin{subfigure}{.32\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{figs/variants_facebook.png} 
  \caption{Facebook}
  \label{fig:variants:others_facebook}
\end{subfigure}
\begin{subfigure}{.32\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{figs/variants_CA-AstroPh.png} 
  \caption{CA-AstroPh}
  \label{fig:variants:others_CA-AstroPh}
\end{subfigure}
\vspace{-3mm}
\caption{Accuracy with and without aligning bases, with nearest neighbor and jv}
\label{fig:variants}
\vspace{-3mm}
\end{figure*}


==> examples/firstpage.tex <==
\begin{figure}[!t]
\centering
\subcaptionbox{Karate club; red edges removed.}[.45\columnwidth]{
\centering
\resizebox{.48\columnwidth}{!}{\input{figs/fp_karate_orig.tex}}
}\hspace{2mm}
\subcaptionbox{Alignment by \thiswork{} (top) and REGAL (bottom).}[.45\columnwidth]{
\centering
\resizebox{.3\columnwidth}{!}{\input{figs/fp_karate_grasp.tex}}
\resizebox{.3\columnwidth}{!}{\input{figs/fp_karate_regal.tex}}
}
%\vspace*{-3mm}
\caption{\pk{With a few removed edges (marked in red), REGAL~\cite{heimann18regal}, the state-of-the-art alignment method based on \emph{local} features, fails to correctly align the distorted Karate club graph to the original; \thiswork (Figure b-top) identifies most of nodes (correctly aligned nodes in green).}}
\label{fig:firstpage}
\vspace{-5mm}
\end{figure}

==> figs/fig-modularity.tex <==
\begin{figure}

\begin{subfigure}{.49\linewidth}
  \centering
  \includegraphics[width=1\linewidth]{figs/cora-modul-DMoN.pdf}  
  \caption{Modularity for DMoN~\cite{tsitsulin2020graph}.}
  \label{fig:modularity:DMoN}
\end{subfigure}
\begin{subfigure}{.49\linewidth}
  \centering
  \includegraphics[width=1\linewidth]{figs/Ucodemodullistcora.pdf}  
  \caption{Modularity for \ourmethod.}
  \label{fig:modularity:UCoDe}
\end{subfigure}


\hspace{-3mm}
\caption{\dmw{Modularity per epoch on Cora dataset. The alternating behaviour \textcolor{blue}{and slightly slower convergence} of \ourmethod is a characteristic of our constrastive loss in Eq.~\ref{eq:objective}, and attains higher overall modularity than DMoN.}}
\label{fig:modularity}
% \vspace{-4mm}
\end{figure}

==> figs/fig-tuning.tex <==

\begin{figure*}
\begin{subfigure}{.33\linewidth}
  \centering
  \includegraphics[width=1\linewidth]{figs/cora-loss-clean.pdf}  
  \caption{\dmw{Loss function on Cora.}} % \cmt{I'm not sure what this caption means -- Andrew}}
  \label{fig:tuning:epochs}
\end{subfigure}
\begin{subfigure}{.33\linewidth}
  \centering
  \includegraphics[width=1\linewidth]{figs/cora-nmi-clean.pdf}  
  \caption{\dmw{NMI (Soft-Cluster) on Cora.}}
  \label{fig:tuning:nmi}
\end{subfigure}
\begin{subfigure}{.33\linewidth}
  \centering
  \includegraphics[width=1\linewidth]{figs/Cora-kmeansdim-nmi-clean.pdf}  
  \caption{Embedding dimension effect on NMI.}
  \label{fig:tuning:dimension}
\end{subfigure}
% \vspace{-1mm}
\caption{\dmw{Study on the impact of parameter settings. \ourmethod correctly minimizes the objective (left), while the quality increases with the number of epochs as desired in (middle). The optimal embedding dimension for the intermediate layer is $256$ (right).}}
\label{fig:tuning}
% \vspace{-4mm}
\end{figure*}





==> tables/tbl-nonoverlapping.tex <==
%!TEX root=../main.tex
\begin{table*}[th]
\newcolumntype{C}{>{\centering\arraybackslash}X}
\newcolumntype{H}{>{\setbox0=\hbox\bgroup}c<{\egroup}@{}}
\begin{tabularx}{\textwidth}{p{2cm}CCCCCCC}
\toprule
Dataset & Kmeans(features) & DGI+kmeans & MinCut  & NOCD & DMoN &\ourmethod(Kmeans)& \ourmethod \\ 
\midrule
Cora  & 15.0 & \uline{55.4} & 37.1 & 43.8 & 46.3 & \textbf{57.3}& 53.5  \\
Citeseer & 22.0 & \textbf{42.5} & 23.1 &  23.9 & 31.4 &  \uline{40.9} & 40.7 \\ 
Pubmed  & \textbf{31.0} & \uline{30.0} & 23.6 & 23.8  & 25.1 & 25.4 & 27.1 \\  
Amazon Photo & 13.6 & 15.6 & - & \uline{61.1} & 55.0 & 59.8 & \textbf{67.0}  \\
Amazon PC & 12.0 & 11.8 & - &\textbf{46.5} & 44.3 &\uline{44.6} & 42.8  \\
Coauthor CS & 33.8 & 67.5 & 68.1 & \uline{73.7} & 67.7 & \uline{78.4}&\textbf{80.2} \\
Coauthor PHY & 20.9 & 51.0 & 45.9 & \uline{57.4}  & 49.8 & 56.3 &\textbf{58.1} \\
\bottomrule
\end{tabularx}
\caption{NMI for non-overlapping community detection results on seven graphs. Best performer in bold; second best underlined.} 
\label{tbl:nonoverlappingrgcn}
\vspace{-6pt}
\end{table*}



\begin{table*}[th]
\newcolumntype{C}{>{\centering\arraybackslash}X}
\newcolumntype{H}{>{\setbox0=\hbox\bgroup}c<{\egroup}@{}}
\begin{tabularx}{\textwidth}{p{2cm}CCCCCCC}
\toprule
Dataset & Kmeans(features) & DGI+kmeans & MinCut  & NOCD & DMoN & \ourmethod(Kmeans) &\ourmethod   \\ 
\midrule
Cora  & 44.1 & \textbf{63.4} & 40.0 & 47.1  & 49.6 & \uline{62.3} & 59.3   \\
Citeseer & 33.8 & \textbf{55.5} & 30.7 & 39.6 & 44.2 & \uline{54.7}& 54.5 \\ 
Pubmed  & 47.9 & \uline{50.3} & 37.2 & 47.5 & 39.1 &\textbf{51.8} & 43.1 \\  
Amazon Photo & 23.4 & 41.2 & - & 57.3 & 57.9 & \uline{59.3}& \textbf{64.2}  \\
Amazon PC & 20.8 & 42.7 & - &\textbf{49.6} & 46.4 & 46.8 &\uline{47.8} \\
Coauthor CS & 41.2 & 59.3 & 58.8 & 66.0 & 58.0 &\textbf{76.8} &\uline{72.8} \\
Coauthor PHY & 41.2 & 30.6 & 47.7 & \textbf{59.1}  & 47.6 & \uline{57.3}& 46.1 \\
\bottomrule
\end{tabularx}
\caption{Fscore for non-overlapping community detection results on seven graphs. Best performer in bold; second best underlined.} 
\label{tbl:nonoverlappingrgcn}
\vspace{-6pt}
\end{table*}



\begin{table*}[th]
\newcolumntype{C}{>{\centering\arraybackslash}X}
\begin{tabularx}{\textwidth}{l*{15}{C}}
\toprule
 & \multicolumn{2}{c}{\cora} & \multicolumn{2}{c}{\citse} & \multicolumn{2}{c}{\pubmed} &
 \multicolumn{2}{c}{\amzph}&
  \multicolumn{2}{c}{\amzpc} &
   \multicolumn{2}{c}{\coacs}&
  \multicolumn{2}{c}{\coaphy}\\
 \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9}
  \cmidrule(lr){10-11} \cmidrule(lr){12-13} \cmidrule(lr){14-15} 
 \textit{method} & $\mathcal{C}$ & $Q$ & $\mathcal{C}$ & $Q$ & $\mathcal{C}$ & $Q$ &$\mathcal{C}$ & $Q$& $\mathcal{C}$ & $Q$ &$\mathcal{C}$ & $Q$ & $\mathcal{C}$ & $Q$  \\  
 \midrule
 kmeans (features)  & 19.0          & 64.0               & 26.1          & 54.2         & 19.7          & 54.2       & 16.9 & 63.7      &  83.0   & 4.0       &   45.9        &   20.9    &       46.0     & 33.3    \\
 DGI+kmeans         &12.4          & 70.7           & 6.13          & 74.4  & 12.4          & 52.7          & 49.3 & 22.4  & 72.0          &  12.6 &   33.6   &    58.6 &    38.6     &   51.2 \\
 
  MinCut             & 22.0          & 70.3            & 11.6          & \textbf{80.9}          & 34.8          & 58.1  &  - & -   & - & - &  \uline{19.8} &       \textbf{72.8} & 28.8   &  62.9 \\
  

NOCD               & 45.1  & \uline{72.2}   &  24.1   &  76.7 &       \textbf{8.3}  & 56.9 & \uline{10.1} & \uline{66.8} & \uline{18.1}       &  \textbf{57.8}          &  20.0         &   72.1      & \textbf{12.9} &  62.2   \\

 DMoN               & 22.3          & 68.1              & \uline{4.6}   & \uline{75.3}        & 17.0          &\textbf{69.2}  & 19.1 & 65.3 & 19.7   &   \uline{55.8}      &  20.0    &\uline{72.3}      & 23.8  &  \textbf{65.8} \\
 
\ourmethod{+}kmeans &\textbf{9.4}   & \textbf{73.9}    & \textbf{4.2}  & 73.2 & \uline{9.4}  & 54.5& \textbf{8.2} & 64.6 &  21.5        &     55.1          &  \textbf{17.5}     &     71.8   &   \uline{14.1}  &    56.1  \\

\ourmethod    &\uline{9.3}    & 71.0  & 5.3           & 73.2  & 13.1  & \uline{59.1}  & 14.7 & \textbf{67.0} & \textbf{17.9}  &   52.8    & \textbf{17.5}     &\swin{72.3}   &  23.5  & \uline{63.1}   \\
\bottomrule
\end{tabularx}
\caption{Graph conductance $\mathcal{C}$ (low is better) and modularity $Q$. Best performer in bold; second best performer underlined.} 
\label{tbl:nonoverlapping-gcn}
\vspace{-6pt}
\end{table*}


























==> tables/tbl-overlapping-recall.tex <==
%\vspace{-2mm}
\begin{table}[!ht]
%\vspace{-4mm}
\small
\newcolumntype{C}{>{\centering\arraybackslash}X}
\newcolumntype{H}{>{\setbox0=\hbox\bgroup}c<{\egroup}@{}}
\begin{tabularx}{\columnwidth}{p{1.4cm}CCCC}
% \toprule
 \cmidrule(lr){1-4} 
 \textit{dataset} & NOCD & DMoN &\ourmethod\\  
 \midrule
Fb-348   & 46.0 & 56.0 & 35.9 \\
Fb-414  & 56.0 &64.0 & 56.3 \\
Fb-686  & 25.3 & 42.7 & 37.1  \\
Fb-698 & 30.5 & 55.2& 42.4 \\
Fb-1684 &44.6& 48.8 & 32.0 \\
Fb-1912 &15.2 & 62.8  & 31.4\\
\eng  & 45.4 & 41.0  & 41.6 \\
\bottomrule
\end{tabularx}
% \vspace{-3mm}
\caption{Recall score results for overlapping community detection results on six graphs} 
\label{tbl:overlapping-recall}
\vspace{-2mm}
\end{table}

==> tables/tbl-overlapping.tex <==
\begin{table}[ht]
\begin{tabularx}{\columnwidth}{lXXXXX}
\toprule
 & Fb-348 & Fb-414 & Fb-686  & Fb-698 & Fb-1684 \\ 
\midrule
BigCLAM  & \uline{26.0} & \uline{48.0} & \uline{13.8}  & \textbf{45.6} & \textbf{32.7}  \\
SNMF & 13.5 & 32.5 &  11.6 & 28.0 & 13.0 \\ 
CDE  & 24.8 & 28.7  & 13.5 & 31.6  & 28.8\\          
EPM & 6.5 & 17.5 & 3.1 & 9.2 & 6.8 \\
\textbf{CoCoDe} & \textbf{28.0} &\textbf{56.0}& \textbf{19.7} & \uline{34.9} & \uline{31.7} \\
\bottomrule
\end{tabularx}
\caption{NMI for overlapping community detection results on four graphs. Best performer in bold; second best underlined.} 
\label{tbl:overlappinggcn}
\end{table} 


==> tables/tbl-ucode-kmeans.tex <==
%!TEX root=../main.tex

\begin{table}[!ht]
%\vspace{-4mm}
\small
\newcolumntype{C}{>{\centering\arraybackslash}X}
\newcolumntype{H}{>{\setbox0=\hbox\bgroup}c<{\egroup}@{}}
\begin{tabularx}{\columnwidth}{p{1.4cm}CCCC}
% \toprule
 & \multicolumn{2}{c}{\textbf{NMI}} & \multicolumn{2}{c}{\textbf{F1}} \\
 \cmidrule(lr){2-3} \cmidrule(lr){4-5} 
 \textit{dataset} & \ourmethodk & \ourmethod & \ourmethodk & \ourmethod \\  
 \midrule
\cora   & 55.4 & 57.4 & 61.1 & 47.5 \\
\citse  & 44.4 & 41.0 & 55.6 & 52.7 \\
\pubmed & 23.5 & 25.0 & 49.3 & 36.1 \\
\amzph  & 61.0 & 67.8 & 52.9 & 66.2 \\
\amzpc  & 38.5 & 44.4 & 36.0 & 49.8 \\
\coacs  & 78.4 & 77.0 & 79.7 & 79.0 \\
\coaphy & 55.3 & 57.5 & 48.5 & 49.0 \\
\bottomrule
\end{tabularx}
% \vspace{-3mm}
\caption{\rev{Comparison between \ourmethod with kmeans clustering on the representations, and \ourmethod.}} 
\label{tbl:ucode-kmeans}
% \vspace{-4mm}
\end{table}


==> tables/tbl_results-nonoverlapping.tex <==



\begin{table*}[th]
\newcolumntype{C}{>{\centering\arraybackslash}X}
\begin{tabularx}{\textwidth}{l*{16}{C}}
\toprule
 & \multicolumn{4}{c}{\textbf{Cora}} & \multicolumn{4}{c}{\textbf{Citeseer}} & \multicolumn{4}{c}{\textbf{Pubmed}} &
 \multicolumn{4}{c}{\textbf{Amazon Photo}} \\
 & \multicolumn{2}{c}{\textit{graph}} & \multicolumn{2}{c}{\textit{labels}} & \multicolumn{2}{c}{\textit{graph}} & \multicolumn{2}{c}{\textit{labels}} & \multicolumn{2}{c}{\textit{graph}} & \multicolumn{2}{c}{\textit{labels}} &
 \multicolumn{2}{c}{\textit{graph}} & \multicolumn{2}{c}{\textit{labels}} \\
 \cmidrule(lr){2-5} \cmidrule(lr){6-9} \cmidrule(lr){10-13} \cmidrule(lr){14-17}
 \textit{method} & $\mathcal{C}$ & $Q$ & NMI & F1 & $\mathcal{C}$ & $Q$ & NMI & F1 & $\mathcal{C}$ & $Q$ & NMI & F1 & $\mathcal{C}$ & $Q$ & NMI & F1 \\  
 \midrule
 kmeans (features)  & 19.0          & 64.0          & 15.0              & 44.1          & 26.1          & 54.2          & 22.0          & 33.8          & 19.7          & 54.2          & \win{31.0} & 47.9 & 16.9 & 63.7 & 13.6 & 23.4  \\
 DGI+kmeans         & 12.4          & 70.7          & \swin{55.4}      & \win{63.4} & 6.13          & 74.4          & \win{42.5} & \win{55.5} & 12.4          & 52.7          & \swin{30.0}  & \swin{50.3} & 49.3 & 22.4 & 15.6 & 41.2\\
 MinCut             & 22.0          & 70.3          & 37.1              & 40.0          & 11.6          & \win{80.9} & 23.1          & 30.7          & 34.8          & 58.1          & 23.6          & 37.2 & - & - & - & -\\
NOCD-X               & 45.1  & \swin{72.2}     & 43.8   & 47.1 &  24.1   &  76.7   &  23.9          & 39.6  &       \win{8.3}  & 56.9          & 23.8 & 47.5 & \swin{10.1} & \swin{66.8} & 61.1 & 57.3 \\
NOCD-G           & 11.5  & 71.3     & 34.8   & 39.8 &  5.5   &  75.5   &  13.5          & 28.9         & 8.7  & 58.7          & 21.8 & 46.6 & 11.0 & 68.3 & 55.0 & 57.9  \\
 DMoN               & 22.3          & 68.1          & 46.3              & 49.6          & \swin{4.6}   & \swin{75.3}  & 31.4          & 44.2          & 17.0          &\win{69.2}  & 25.4          & 39.1 & 19.1 & 65.3 & 59.3 & 55.7 \\
\ourmethod(soft)    &\swin{9.3}    & 71.0  & 53.5              & 59.3          & 5.3           & 73.2          & 40.7          & 54.5          & 13.1  & \swin{59.1}  & 27.1          & 43.1 & 14.7 & \win{67.0} & \win{67.0} & \win{64.2} \\
\ourmethod{+}kmeans &\win{9.4}   & \win{73.9} & \win{57.3}   & \swin{62.3}    & \win{4.2}  & 73.2          & \swin{40.9}  & \swin{54.7}  & \swin{9.4}  & 54.9          & 25.1          & \win{51.8} & \win{8.2} & 64.6 & \swin{59.8} & \swin{59.3} \\
\bottomrule
\end{tabularx}
\caption{Results on four datasets in terms of graph conductance $\mathcal{C}$ (low is better), modularity $Q$, NMI with ground-truth labels, and pairwise F1 measure. Best performer in bold; second best performer underlined.} 
\label{tbl:nonoverlapping-gcn}
\vspace{-6pt}
\end{table*}



%%% The results are from Anton's paper %%%
\begin{table*}[th]
\newcolumntype{C}{>{\centering\arraybackslash}X}
\begin{tabularx}{\textwidth}{l*{16}{C}}
\toprule
 & \multicolumn{4}{c}{\textbf{Amazon PC}} & \multicolumn{4}{c}{\textbf{Coauthor CS}} & \multicolumn{4}{c}{\textbf{Coauthor PHY}} &
 \multicolumn{4}{c}{\textbf{}} \\
 & \multicolumn{2}{c}{\textit{graph}} & \multicolumn{2}{c}{\textit{labels}} & \multicolumn{2}{c}{\textit{graph}} & \multicolumn{2}{c}{\textit{labels}} & \multicolumn{2}{c}{\textit{graph}} & \multicolumn{2}{c}{\textit{labels}} &
 \multicolumn{2}{c}{\textit{graph}} & \multicolumn{2}{c}{\textit{labels}} \\
 \cmidrule(lr){2-5} \cmidrule(lr){6-9} \cmidrule(lr){10-13} \cmidrule(lr){14-17}
 \textit{method} & $\mathcal{C}$ & $Q$ & NMI & F1 & $\mathcal{C}$ & $Q$ & NMI & F1 & $\mathcal{C}$ & $Q$ & NMI & F1 & $\mathcal{C}$ & $Q$ & NMI & F1 \\  
 \midrule
 kmeans (features)  &  83.0   & 4.0  &   12.0        &   20.8        &   45.9        &   20.9      &        33.8   & 41.2  &     46.0     & 33.3  & 20.9 & 41.2 & &  &   \\
 DGI+kmeans     & 72.0          &  12.6  &  11.8         &  42.7        &   33.6   &    58.6     &  67.5          & 59.3          &     38.6     &   51.2 &  51.0  &  30.6 &  & &  &   \\
 MinCut    & - & - & - & -  & \textbf{19.8} &       \win{72.8}    & 68.1   &  58.8  & 28.8   &  62.9 & 45.9  & 47.7 &    & &  &   \\
NOCD-X   & \swin{18.1}       &  \win{57.8}        &   \win{46.5}          &   \win{49.6}        &  20.0         &   72.1      & 73.7     &  66.0 &   \win{12.9} &  62.2   &  \swin{57.4} & \win{59.1}  &  & &  &   \\
NOCD-G       & 23.8          & 60.9          &  42.7           &   42.3  &  19.7    &   72.8      &   66.8        &     60.6      &          &          &  &  &  & &  &   \\
 DMoN     & 19.7   &   \swinf{55.8}    &    44.3       &  46.4           &  20.0    &\swin{72.3}     &      67.7     & 58.0      & 23.8  &  \win{65.8} &   49.8   &  \textbf{47.6} &  &  & &  
 \\
\ourmethod(soft)  & \win{17.9}  &   52.8  &   42.8         &  \swin{47.8}         & \win{17.5}     &\swin{72.3}    &  \win{80.2}     &   \swin{72.8}      &  23.5  & \swin{63.1}   & \win{58.1} &   46.1  & &  &  & \\
\ourmethod{+}kmeans &  21.5        &     55.1      & \textbf{44.6}         &     46.8         &  \win{17.5}     &     71.8   &\swin{78.4}     & \win{76.8}  &   \swin{14.1}  &    56.1     &56.3 & \swin{57.3} &  & &  &   \\
\bottomrule
\end{tabularx}
\caption{Results on four datasets in terms of graph conductance $\mathcal{C}$ (low is better), modularity $Q$, NMI with ground-truth labels, and pairwise F1 measure. Best performer in bold; second best performer underlined.} 
\label{tbl:nonoverlapping-gcn}
\vspace{-6pt}
\end{table*}



